Classification of multivariate weakly-labelled time-series with attention

This research identifies a gap in weakly-labelled multivariate time-series classification (TSC), where state-of-the-art TSC models do not per-form well. Weakly labelled time-series are time-series containing noise and significant redundancies. In response to this gap, this paper proposes an approach of exploiting context relevance of subsequences from previous subsequences to improve classification accuracy. To achieve this, state-of-the-art Attention algorithms are experimented in combination with the top CNN models for TSC (FCN and ResNet), in an CNN-LSTM architecture. Attention is a popular strategy for context extraction with exceptional performance in modern sequence-to-sequence tasks. This paper shows how attention algorithms can be used for improved weakly labelledTSC by evaluating models on a multivariate EEG time-series dataset obtained using a commercial Emotiv headsets from participants performing various activities while driving. These time-series are segmented into sub-sequences and labelled to allow supervised TSC.

==> backup/backup_main.tex <==
% % It is an example file showing how to use the 'sigkddExp.cls' 
% % LaTeX2e document class file for submissions to sigkdd explorations.
% % It is an example which *does* use the .bib file (from which the .bbl file
% % is produced).
% % REMEMBER HOWEVER: After having produced the .bbl file,
% % and prior to final submission,
% % you need to 'insert'  your .bbl file into your source .tex file so as to provide
% % ONE 'self-contained' source file.
% %
% % Questions regarding SIGS should be sent to
% % Adrienne Griscti ---> griscti@acm.org
% %
% % Questions/suggestions regarding the guidelines, .tex and .cls files, etc. to
% % Gerald Murray ---> murray@acm.org
% %

% \documentclass{sigkddExp}

% \input{packages.tex}

% \graphicspath{ {./images/} }

% \def\cw#1{\textcolor{blue}{#1}}

% \begin{document}
% %
% % --- Author Metadata here ---
% % -- Can be completely blank or contain 'commented' information like this...
% \conferenceinfo{ACM Sigkdd}{Singapore} % If you happen to know the conference location etc.
% %\CopyrightYear{2001} % Allows a non-default  copyright year  to be 'entered' - IF NEED BE.
% %\crdata{0-12345-67-8/90/01}  % Allows non-default copyright data to be 'entered' - IF NEED BE.
% % --- End of author Metadata ---

% \title{Classification of multivariate weakly-labelled time-series with attention}
% %\subtitle{[Extended Abstract]
% % You need the command \numberofauthors to handle the "boxing"
% % and alignment of the authors under the title, and to add
% % a section for authors number 4 through n.
% %
% % Up to the first three authors are aligned under the title;
% % use the \alignauthor commands below to handle those names
% % and affiliations. Add names, affiliations, addresses for
% % additional authors as the argument to \additionalauthors;
% % these will be set for you without further effort on your
% % part as the last section in the body of your article BEFORE
% % References or any Appendices.

% \numberofauthors{1}
% %
% % You can go ahead and credit authors number 4+ here;
% % their names will appear in a section called
% % "Additional Authors" just before the Appendices
% % (if there are any) or Bibliography (if there
% % aren't)

% % Put no more than the first THREE authors in the \author command
% %%You are free to format the authors in alternate ways if you have more 
% %%than three authors.

% \author{
% %
% % The command \alignauthor (no curly braces needed) should
% % precede each author name, affiliation/snail-mail address and
% % e-mail address. Additionally, tag each line of
% % affiliation/address with \affaddr, and tag the
% %% e-mail address with \email.
% \alignauthor Surayez Rahman \\
%       \affaddr{Faculty of Information Technology}\\
%       \affaddr{Monash University, Clayton Campus}\\
%       \affaddr{Melbourne, Australia}\\
%       \email{srah0001@student.monash.edu}
% \alignauthor Chang Wei Tan\\
%       \affaddr{Faculty of Information Technology}\\
%       \affaddr{Monash University, Clayton Campus}\\
%       \affaddr{Melbourne, Australia}\\
%       \email{chang.tan@monash.edu}
% \alignauthor Mahsa Salehi\\
%       \affaddr{Faculty of Information Technology}\\
%       \affaddr{Monash University, Clayton Campus}\\
%       \affaddr{Melbourne, Australia}\\
%       \email{mahsa.salehi@monash.edu}
% }

% \date{06 November 2020}

% \maketitle
% \begin{abstract}
% This paper provides a sample of a LaTeX document for final submission
% to Sigkdd Explorations, the official newsletter of ACM Sigkdd. This is
% a modified version of the ACM Proceedings sample file.

% The developers have tried to include every imaginable sort
% of ``bells and whistles", such as a subtitle, footnotes on
% title, subtitle and authors, as well as in the text, and
% every optional component (e.g. Acknowledgements, Additional
% Authors, Appendices), not to mention examples of
% equations, theorems, tables and figures.

% To make best use of this sample document, run it through \LaTeX\
% and BibTeX, and compare this source code with the printed
% output produced by the dvi file.

% To make best use of this sample document, run it through \LaTeX\
% and BibTeX, and compare this source code.
% \end{abstract}

% \section{Introduction}
% Time-series classification \cw{(TSC)} is one of the most well-researched areas of modern computer science \cite{Bagnall2017-xw}. 
% \cw{With the increase in time series data, accurate real-time TSC has become more important than ever.}
% % With the rise in time-series data analysis, real-time time-series classification is a very important concept in the current world scenario. 
% Despite the huge progress in \cw{TSC} over the last decade \cite{Bagnall2017-xw}, most of these works make assumptions that are unrealistic in the real-world setting. 
% This includes the assumption that the patterns (subsequences) that exist in the time-series are of fixed equal lengths and are always correctly labelled \cite{Hu2016-go}. 

% However, in the real-world settings, these patterns can be of unequal length, the class label of the pattern may contain errors and may only correspond to a general section of the data.
% \cw{This is commonly known as \emph{weakly labelled} data \cite{Hu2016-go}.}
% % More importantly, the class labels are typically highly imbalanced. 
% % and filled with noise or other redundancies, as will be shown in this paper.
% % To illustrate an example
% \cw{For instance}, Figure \ref{fig:eeg} shows \cw{a sample of weakly labelled Electroencephalography (EEG) signal}
% obtained from a participant during driving using \cw{the} Emotiv Epoc+ EEG headset \footnote{\url{https://www.emotiv.com/epoc/}}. 
% The 14\cw{-channel EEG signal can be interpreted as a time series with 14 dimensions.
% Then a time series analysis algorithm can be applied to analyse the brain waves of the driver and detect the state of the driver, either focused or distracted.} 
% % time-series here are captured simultaneously and each of them represents a single channel of EEG brain signals.
% \cw{The different colors as indicated in the legend represent the different activities during driving.
% These activities are weakly labelled because it is challenging to correctly label driver's transition from driving to using an iPad and vice versa.
% Besides, these subsequences may also contain noise or redundant patterns that are not related to the activity that driver is performing at that point in time.
% In fact, these redundant patterns may occur in different activity patterns, which is challenging to differentiate the different activities.}
% % \cite{noauthor_undated-rv}.
% % , where the x-axis represents time, the y-axis signifies fluctuations in brain signals. 
% % Each sequence is coloured to represent different activities during driving as shown in the legend.
% % When collected raw, the data are not labelled as such and there are no distinct points to when the driver transitions from driving to using an iPad. The only annotation given for this data is that it represents brain signals of a driver who is generally focused. 
% % \cw{Typically}, in such \emph{weakly labelled} time-series, each \cw{subsequence tend to be} very similar to the other \cw{subsequences, even when they have different labels. 
% % This makes it extremely challenging to differentiate the subsequences of different labels.}
% % due to the overlay of recorded noise and each sequence are of varying lengths. 
% % Typically such time-series are highly imbalanced such that they contain much more driving data than distracted data.
% % Moreover, such multivariate data can only make sense if these parallel time-series are analysed together and therefore, it elevates the difficulty for algorithms to consume and build an understanding of the data.

% \begin{figure}[t]
% % \centering
% \includegraphics[width=\linewidth]{.images/Emotiv14.png}
% \caption{Example of a weakly labelled EEG data}
% \label{fig:eeg}
% \end{figure}


% \cw{Moreover, most real-world time series dataset such as the example in Figure \ref{fig:eeg} are  highly imbalanced where they contain more of the ``normal'' label and multivariate in nature.
% In this case, there are more driving labels than distracted labels, thus making the task of predicting a distracted activity extremely challenging.}
% % Typically such time-series are highly imbalanced such that they contain much more driving data than distracted data.
% % Moreover, such multivariate data can only make sense if these parallel time-series are analysed together and therefore, it elevates the difficulty for algorithms to consume and build an understanding of the data.



% For time-series classification, Fully Convolutional Network (FCN) and Residual Network (ResNet) are two state-of-the-art deep learning algorithms \cite{Ismail_Fawaz2019-tc}, but unfortunately, when these models were evaluated in this research, they demonstrated poor accuracies in classifying multivariate weakly-labelled time-series. It makes sense because these models were designed to extract and interpret features from individual sequences to classify their category. While this strategy works well for noise-free time-series with proper annotations, it fails to extract discriminative features from weakly-labelled time series as it cannot distinguish between noise and useful data, especially when the class labels are highly imbalanced.

% This research identifies a requirement to develop generalised supervised-neural-network models that can accurately classify multivariate weakly-labelled time-series in real-time. The approach explores the use of ‘attention’ strategy \cite{Bahdanau2014-eh} to extract the contextual relevance of sequences, using which noise and redundancies from data can be eliminated during classifications. The intuition behind this is the chronological order of time-series, such that under realistic conditions, they follow certain chronological trends. For example, in the EEG time-series, the data will typically show a driver who is distracted at one moment has a higher probability of being distracted in the next moment or show gradual changes, rather than a sudden spike in concentration levels.

% Therefore, this research studies a set of deep learning models that can classify each sequence of time-series and understand sequence correlations using attention to resolve noise. The attention models are adapted from original designs in the field of NLP and are implemented within existing state-of-the-art deep learning models to classify weakly labelled multivariate in real-time with better performance than existing models.



% \section{Background and Related Work}


% The field of time-series classification (TSC) has advanced significantly in the last decade, with each of them being significantly more accurate than its predecessors. The following section outlines the strength and limitations of some of the existing state-of-the-art TSC algorithms.

% \subsection{State-of-the-art TSC Algorithms}

% In 2020, Dempster et. al. \cite{Dempster2020-ck} proposed an algorithm called ROCKET, that extracts features from the time series using random convolutional kernels for uni-variate time series classification in real-time. ROCKET is scalable and achieves state-of-the-art performance in time series classification. It can easily be adapted for multivariate data with similar performance. This research applies ROCKET on weakly-labelled multivariate time series, however as shown later, the performance of the model is not high enough, particularly on time-series containing large quantities of noise and redundancies. This was expected as ROCKET was not designed to classify weakly labelled time-series. In fact, none of the state-of-the-art time-series classification algorithms is designed to classify weakly labelled time-series in real-time.

% Previously in 2019, Ismail et. al. \cite{Ismail_Fawaz2019-tc} evaluated two state-of-the-art deep-learning models, Fully Connected Network (FCN) and Residual Network (ResNet), for TSC. FCN and ResNet are deep-learning convolutional neural-networks, that extract features from time-series by generating a set of feature-maps. ResNet has residual connections that further help it reduce any vanishing gradient effect \cite{Hochreiter1998-uf}.


% % The architecture for these two models are important to this study and are discussed below in detail.
% % Maybe we can skip the description about FCN and ResNet?
% % \cw{\subsubsection{Fully Convolutional Network (FCN)}}

% % \cw{The FCN model is designed with three convolutional blocks and a final Global Averaging Pool (GAP) layer. The first convolution block creates a set of feature-maps and then passes it on to the next block. Each feature map is a representation of various features learnt by the model for a sequence. The next two blocks further improve and update these feature-maps, and pass them to the GAP layer. The GAP layer takes the average pooling of the features, on which a softmax function is applied in the final dense layer to determine the class of the sequence.}

% % \cw{\subsubsection{Residual Network (ResNet)}}

% % \cw{ResNet is designed with nine convolutional neural blocks, which work similar to the FCN model, and includes an additional ability to take ’shortcuts’ using residual connections. These shortcuts escalate the model to learn and classify very quickly and help the model reduce the vanishing gradient effect. In some time-series, the changes in data are very small, which means their learning gradient is extremely small. While a general neural model learns these changes negligibly, with the help of residual connections, ResNet can overcome these inaccuracies. This is important in this study because it prevents inaccurate training on weakly labelled time-series that have tiny variations. Finally, ResNet has a GAP layer at the very end that enables the model to generally work well across a variety of time-series data.}

% Both of these neural network models can classify multivariate time-series in real-time, but they were designed to classify clean and processed time-series, unlike in a real-world setting.  When these models were evaluated as is in this research, their performance metrics were not exceptional on weakly labelled data, as will be shown later in the paper. 

% In 2019, Perslev et. al. \cite{Perslev2019-db} introduced an advanced segmentation algorithm called U-Time, which uses a feed-forward network with convolutional encoders and decoders to segment sequences of long time-series. U-Time demonstrated high segmentation accuracy on a range of multivariate weakly labelled time series such as real-life sleep-staging time-series. The model can be expected to classify multivariate weakly labelled time-series successfully, however, due to the nature of feed-forward networks, complete input time-series must be provided to the model before it can segment or classify each sequence of the time-series. This is a drawback for real-time classification where data will be streamed continuously and the model would need to analyse new prevailing sequences. For real-time analysis, U-Time would become computationally expensive and hence, U-Time is not the most appropriate model out of the box. However, U-time can be explored in future to apply the intuition for real-time time-series classification.

% ROCKET, FCN, ResNet and U-Time are among the most recent and advanced multivariate time-series analysis models, but none are designed to interpret weakly labelled data correctly in real-time. Therefore, this research identifies the lack of a proper neural network model to classify multivariate weakly-labelled time-series in real-time with high-performance metrics.

% Among these existing state-of-the-art models, this research focused on FCN and ResNet because their neural network architecture allows them to be upgraded. If these models can remove noise and redundancies of weakly labelled data, they will be able to drastically improve their performance scores. One of the ways of doing this efficiently is to learn the contextual relevance of the sequences. Expanding on this idea, this research introduces the attention mechanism to allow deep learning models to get a comprehensive understanding of the context of input time-series.


% \subsection{Attention}

% The attention concept was initially proposed in 2015 by Bahdanau et. al. to utilise the contextual information in sequence-to-sequence (Seq2Seq) problems such as natural language processing (NLP) \cite{Bahdanau2014-eh}. Seq2Seq are neural networks that consume and output continuous sequences of data. These models are typically encoder-decoder architectures, where the encoders consume the complete input sequences before decoding the output sequence. When input sequences are long, generating the contextual information becomes a bottleneck. To prevent this problem, this attention strategy was introduced to decouple the encoders and decoders to allow long sentences to be translated accurately using bi-directional alignment functions.

% Since then, several other designs of attention were introduced by several following papers, mostly focused on NLP. Subsequently, in 2015, Luong et. al \cite{Luong2015-xr} proposed an attention strategy with an encoder-decoder architecture. The language translation model was based on the intuition to keep track of all the words in a sentence so that the relevance of each word to the current word can be used to make better translation decisions. This attention uses multiple calculations to derive the context and is faster than the initial model by Bahdanau et. al.

% Self-Attention and Multi-Head Attention are two state-of-the-art attention models in NLP proposed by Vaswani et. al. \cite{Vaswani2017-xw} in 2017. These models build correlation functions using neural networks and use a complex encoder-decoder architecture, known as the Transformer \cite{Vaswani2017-xw}, to learn the trends of sequence to sequence data. Since then, these models have been used in the research of various problem domains \cite{Weng2018-fc} to leverage the relevance of sequence-to-sequence data. 

% For this research, the above-mentioned set of attention strategies, which were originally built for NLP, are studied thoroughly. This study recreates these models with LSTM encoders and decoders to allow them to understand and interpret the context of time-series data. Hence, the architecture and flow of these models are described in detail in the following sections.


% \section{Methodology}
% \cw{CW: I think it is better to have this section organised in this way. Start with some motivation that FCN or typical TSC algorithms failed (point to the results section), then talk about encoder decoder structure where we use FCN-LSTM etc and finally add attention to it.}

% Relevance information in TSC are additional context such as 'two previous sequences from a same category have sections that show similar patterns as the current sequence'. When the existing supervised neural-networks are incorrectly learning the distinctive features from sequences because of noise or erroneous data, additional context can help the models identify similar sections of a sequence to previous sequences to correctly identify its category.

% This means, even if the current sequence is much longer or shorter in length, finding sections relevant to previous sequences would help the model understand the correct category of the sequence, therefore eliminating the effect of sequence length. Similarly, if the data is imbalanced and the model does not have enough data to learn the features of the minority category, the contextual information can tip the classification decision for a sequence towards the correct category, as soon as it detects relevant sections with previous sequences belonging to that minority category.

% Since time-series data follow continuous order, the level of noise or redundancy is expected to show continuous changes. If the model can constantly keep track of the noises and redundancies by comparing the relevance of sections from previous sequences, it can continuously learn and cancel out the effect of noise or redundancies. This intuition highlights two aspects of a desired neural network in this research; it must be supervised to allow the model to learn features corresponding to categories correctly and secondly, it must be able to keep track of the contextual information for every sequence with its previous ones. Therefore, using the state-of-the-art supervised models FCN and ResNet, various context-extraction strategies, including LSTM and attention, are experimented in this research. 


% \subsection{The Encoder-Decoder}

% To allow context extraction from previous sequences, multiple sequences need to be passed to the models per batch. In this research, four sequences are passed per batch so that the models can use the first three sequences to extract context, and the feature-maps from FCN or ResNet, to categorise the final sequence in the batch. Exactly four sequences are used so that the maximum contextual information of nearest neighbours can be retained with the highest priority. Passing more sequences can negatively impact context extraction as it introduces the problem of ‘vanishing gradient’ \cite{Hochreiter1998-uf} on RNN, where the oldest context stored by the model fade away as new data are inserted.

% The existing implementations of FCN and ResNet can accept single sequences. Therefore, to allow multiple sequences to be processed, an encoder-decoder architecture is introduced.

% \subsubsection{Architecture}

% When deep learning layers receive four sequences together in a batch, they create a single set of feature-maps for the complete length of the input time-series. These feature-maps are not useful if they are directly passed to an attention layer because attention cannot segment the feature-maps for each sequences. To prevent this, a Time-Distributed layer from the Keras library is introduced after the deep learning layers. The time-distributed layer acts as a wrapper that slices the feature-maps into four sections for each sequence, and passes them onto an LSTM encoder. LSTM can retain small blocks of data and the encoders use it to store the feature-maps received for the four sequences from FCN or ResNet.

% \begin{figure}[h]
% \centering
% \includegraphics[width=6cm]{.images/enc-dec.png}
% \caption{Encoder-Decoder architecture}
% \end{figure}

% The encoder receives these four separated set of hidden states and passes them onto the next layers. This is where context-extraction strategy can be implemented. The four set of hidden states can be used to extract contextual information to return a context vector. The encoder will then concatenate the context vector received with the four set of hidden states and pass these on to the decoder. The LSTM decoder can unwrap the encoding to make sense of the feature-maps, and pass it onto the output layer to classify the last sequence.


% \subsection{LSTM Approach}

% This research evaluates the performance by FCN and ResNet with just the LSTM layers to extract basic context. LSTM are RNNs that have 

% Following up on LSTM approach, a set of attention strategies are implemented to evaluate performance changes for TSC.

% \subsection{Attention Approach}

% The attention strategies studied in this research are well-established state-of-the-art context-extraction models, typically for seq-2-seq analysis such as NLP. Specifically, this research recreates the following existing attention strategies and combines them with FCN and ResNet to experiment with performance for weakly labelled TSC.

% \begin{enumerate}[leftmargin=*]
%   \setlength\itemsep{0.2em}
%   \item Alignment Attention, introduced by Luong et. al. \cite{Luong2015-xr}
%   \item Bi-directional Attention, by Bahdanau et. al. \cite{Bahdanau2014-eh}
%   \item Locally and Globally focused Self-Attention Model, designed by Vaswani et. al. \cite{Vaswani2017-xw}
%   \item Multi-Head Attention Model, also by Vaswani et. al. \cite{Vaswani2017-xw}
% \end{enumerate}

% The next few sections describe the architecture of the existing attention and the benefits of the components with regards with TSC.

% \subsubsection{Luongs' Attention}

% With the potential to weigh the relevance of neighbouring sequences, this research adopts the idea of attention from Luong et. al. \cite{Luong2015-xr} and re-creates the attention model to accept time-series data. Since the original model is designed for language translation data, to allow time-series training and classification, the original model required several structural changes. Therefore, this study followed an implementation concept proposed by Huangwei \cite{Wieniawska2020-cv}.

% In the original architecture, the model was built with twenty individual encoders and decoders. For this study, exactly four encoders and decoders are used such that in each batch, exactly four sequences are accepted and processed by the model. 

% In every batch, the four input sequences are distributed to each of the four LSTM encoders in order. The idea is to classify the very last sequence based on the sequence-relevance information from the previous three sequences.

% \begin{figure}[h]
% \centering
% \includegraphics[width=6cm]{.images/Luong.png}
% \caption{Luongs' attention to process time-series}
% \end{figure}

% The encoders return a set of ‘hidden-states’ which are in fact feature-maps that are trained to understand and hold various features of the sequences. Since the last encoder hidden-state is responsible for the classification of the last (currently focused) sequence, this hidden-state is passed onto the decoder which repeats the vector four times to initiate a series of hidden decoder states.

% A dot product layer is applied to the encoder and decoder hidden-states which creates a series of context vectors, each containing alignment scores. These alignment scores represent how well each of the first three sequences matches with the features extracted from the last sequence. But to get a decodable weight value, the alignment scores are again multiplied with the last hidden state from the encoder and a weighted sum is calculated. Using these weights, the decoder understands how well the last sequence is relevant to the previous sequences and how previous patterns in the sequence are followed through in the last sequence. 

% These decoder states can now be used by any deep learning model to suave their feature-maps towards the correct category in case the deep learning feature-maps are incorrectly guided due to noise and redundancies.

% \subsubsection{Bi-directional Alignment Attention}

% The strategy suggested in the paper by Bahdanau et. al., is that the trend of data can be better understood if the pattern is analysed in order and reverse. While it is useful to understand the relevance of previous sequences affecting the next ones, it can also be beneficial to know how the class of a previous sequence might be affected based on the classification made on the current sequence.

% Following this concept of analysing data trends in both directions, this research implements a bi-directional encoder system on the existing Luongs' implementation to better understand the relevance of sequences. However, it is important to note that exactly four sequences are passed to this model per batch (similar to the previous implementation) to correctly classify the final sequence.

% This attention model is implemented with a similar design as the previous model with some major changes in the encoders.

% The model begins by receiving a batch of four time-step data into the encoder. To allow analysis in both directions, a bi-directional RNN (LSTM) is used to learn the representation of the input sequence in order and backwards. Each direction of the LSTM encoder creates a set of hidden states, labelled in the following flow chart as [E1, E2, E3, E4] and [B1, B2, B3, B4] for forwards and backwards respectively. These hidden states represent the alignment scores, similar to the previous model, but individually for each direction.

% \begin{figure}[h]
% \centering
% \includegraphics[width=8cm]{.images/BiDirectional.png}
% \caption{Bi-Directional attention for time-series}
% \end{figure}

% These hidden states are then concatenated such that each of them collectively determines the overall alignment score in both forward and backward directions.

% Finally, the decoder uses these sets of alignment scores to assign a weight of each of the first three sequences on the last one, representing how well the sequence follows features from the previous sequences.


% \subsubsection{Transformers}

% While the models by Luong et. al. \cite{Luong2015-xr} and Bahdanau et. al. \cite{Bahdanau2014-eh} can train and classify based on preceding sequences, two transformer designs, Self-Attention and Multi-Head Attention, are also evaluated in this research.

% Both these transformer models \cite{Vaswani2017-xw} have built-in stacks of encoders and decoders, where each encoder is identical to the others and the same applies to the decoders. Generally, these encoders are designed as a bundle containing an Attention layer and a Feed-Forward Neural Network (FFNN). 


% \begin{figure}[h]
% \centering
% \includegraphics[width=7cm]{.images/transformer.png}
% \caption{Transformer Enc-Dec architecture}
% \end{figure}


% The Attention layer can be tweaked as necessary but generally, a Self-Attention layer (discussed later) is applied. The encoders and decoders contain internal residual connections, that are responsible for quick and adaptive feature extraction. The specific design features and advantages of this transformer architecture are further discussed in the next two sections where it is used within the Self-attention and Multi-Head Attention models.

% \subsubsection{Self-Attention}
% The core Self-Attention library implemented in this study was adapted from a Keras implementation by CyberZHG \cite{Zhao_undated-at}, built together with LSTM encoder and decoder to process time-series.

% Two different streams of Self-Attention were implemented as part of this study. Initially discussed in the papers by Bahdanau et. al and Luong et. al, the concept of hard vs. soft attention drives the design for each of these streams. Soft attention is a strategy to calculate alignment weights ‘softly’ across a group of input sequences, focusing on the overall trend. On the other hand, hard attention aggressively focuses on specific areas of input sequences and therefore, learns to identify definite features in each sequence.

% This gives rise to the concept of global and local self-attention models. The global self-attention implemented in this research leverages the soft attention strategy to learn overall patterns across all the previous sequences, whereas local attention is a careful balance of both hard and soft attention. In a local self-attention implementation, the hard attention concept is primarily used to predict a single alignment score for the current sequence using feature-maps as described in the alignment models, then the soft attention creates a context vector of a window centred around the position of the current sequence. This window stretches along with the group of input sequences so the model gets an overall perspective of the trend.

% Self-Attention uses transformer encoders and decoders as defined in the previous section. The underlying concept of these models utilises matrices to keep track of context. For each sequence of the input time-series, the encoder generates three different vectors: Query, Key and Value vectors using the output from the LSTM encoder.

% Firstly, an alignment score for each sequence is calculated, which is the dot product of the query and key vectors for each sequence. A softmax layer is used to normalise these series of alignment scores to reveal the weight of each sequence suited towards a particular category, also known as softmax scores. 

% The model can simply predict the category of each sequence based on the maximum softmax score for each sequence, but it proceeds to an additional step. For each sequence, it multiplies the initially created value vector with the softmax scores. This creates a filter to extract the previous sequences that are more relevant to the current sequence than others, which are now completely diminished. This extra feature allows the model to flush out irrelevant previous sequences more smartly, and therefore ignore any noise or redundancies of previous sequences that can affect the classification of the last one.

% The resulting scores can now be summed up to find the highest weight that corresponds to a category. However, the transformer decoders use these weights to further align and refine them through its self-attention and FFNN layers to finally determine a category for each sequence at the output layer.

% In this study, the performance of two different alignment score functions of self-attention is evaluated. These additive and multiplicative functions were discussed in the original paper \cite{Vaswani2017-xw}.

% The additive function calculates the scores by passing the query(Q), key(K) and value(V) vectors to a hidden layer of a Feed-Forward Network (FFN) and decoding its output. On the contrary, multiplicative functions pass the vectors into a softmax layer where the scores are calculated as equation 1 below. Here, dk refers to the dimensions of the vector K, which are representations of hidden states from the encoder.

% \begin{equation}Attention(Q, K, V)=softmax(\frac{QK^T}{\sqrt{d_k}})V\end{equation}

% According to the paper \cite{Ismail_Fawaz2019-tc}, the additive function is expected to outperform multiplicative function when the encoder key dimension, dk, is large. The encoder key dimension depends on how complex the input time-series sequences are if there are more features to learn from the sequence, the dimensions are higher and vice versa. In the case of multiplicative (dot-product) approach, large dk means scores grow in higher magnitudes and therefore extreme gradient values are generated. However, the division of softmax scores by root of dk stalls this problem. Assuming that the complexity of the input time-series is not definitive, this research evaluates the self-attention strategy in both multiplicative and additive schemes.

% \subsubsection{Multi-Head Attention}
% Multi-Head Attention (MHA) is a strategy which adapts the idea of self-attention previously discussed, however, at the cost of high computation power during training, it runs several self-attention models together to perform classification. In this research, Multi-Head Attention is implemented primarily based on a Keras library by CyberZHG \cite{Zhao_undated-at}. However, improvements are made on this model based on the implementation of the original paper \cite{Vaswani2017-xw}, which is now available as a Tensorflow library \cite{noauthor_undated-sg}. Together with the transformer encoders and decoders, the Multi-Head Attention implemented in this research can support weakly-labelled time-series classification.

% Similar to the self-attention model, the implemented Multi-Head Attention (MHA) model is also given a set of four sequences per batch, to classify the last one. The model initially creates three vectors: key (K), value (V) and query (Q), but these sets of vectors are replicated ‘h’ times, where h is the number of heads selected as a hyper-parameter. This h value decides how many self-attention models will be running in parallel where each self-attention receives its own set of K, V and Q vectors.

% The encoder designs are similar to the previously discussed Self-Attention encoders. However, the attention layer of the encoders in MHA will run ‘h’ parallel self-attentions within each encoder and a combined output of these will be passed into the next FFNN.

% Each of the attention heads individually run dot-product self-attention, then concatenate all their K, V and Q vectors to a single set of each before passing them on. This ensures that each position within the encoder can attend to all positions of the previous layers, therefore building more context as it passes to the next encoder.

% The parallel attentions help the encoders understand the relevance of multiple areas of input sequences at the same time. The diagram below shows how the last sequence is relevant to two previous sequences but not to the first one. MHA allows the model to focus on individual positions within these two previous sequences to make further classification decisions, and at the same time flushes out the irrelevant ones based on the filtration by self-attention discussed before.

% \begin{figure}[h]
% \centering
% \includegraphics[width=8cm]{.images/MHA.png}
% \caption{MHA focus on time-series sequence positions}
% \end{figure}

% While these multi heads allow parallel focus on multiple sequences, time-series sequences need to consider the order. It is only useful for the model to keep track of neighbouring sequences if they follow any specific trend. MHA takes care of the order by an additional vector known as positional encoding. This keeps track of the distance between each sequence, giving the model a sense of sequence order. These vectors are added to the initial encoded inputs to allow the next encoders and decoders to utilise this to make sense of order.

% The decoders are masked such that they only consider previous sequences before making current predictions. This is important in this study because it enables the model to suit real-time classifications where future sequences are not known. While the previous models also follow this restriction, MHA requires this additional masking due to multiple Self-Attention running in parallel and MHA cannot control individual attention encoder/decoder centrally.

% As the model steps through all the decoders, a set of probability scores are returned from a softmax layer that helps the model determine which classification has the highest probability. This is very similar to the strategy followed by general self-attention models.

% \subsection{The Deep learning Attention Models}
% \cw{CW: how is this section different from previous section? Attention is also a deep learning model}

% The deep-learning models, FCN and ResNet, are designed to learn features of a sequence and classify them into a category, whereas attention models are designed to extract the context of each sequence with its previous sequences. To take advantage of both the strategies, this research combines the attention mechanisms with deep learning models. While most of the attention strategies discussed above are integrated with either FCN or ResNet, some of them are built independently to evaluate individual performance.



% \subsection{Multi-Step Models}

% Since this architecture of deep learning with attention models are designed to receive four sequences per batch, these models can be categorised as multi-step models. The list of the multi-step models implemented in this research include:

% \begin{itemize}
%   \setlength\itemsep{0.2em}
%   \item \textbf{FCN\_LATTN}: Luong’s Attention with FCN
%   \item \textbf{ResNet\_LATTN}: Luong’s Attention with ResNet
%   \item \textbf{FCN\_BATTN}: Bahdanau’s Attention with FCN
%   \item \textbf{ResNet\_BATTN}: Bahdanau’s Attention with ResNet
%   \item \textbf{SelfA}: Local Additive Self-Attention
%   \item \textbf{FCN\_SelfA}: Local Additive Self-Attention with FCN
%   \item \textbf{FCN\_SelfA\_Global}: Global Self-Attention with FCN
%   \item \textbf{FCN\_SelfA\_Multiplicative}: Local Multiplicative Self-Attention with FCN
%   \item \textbf{ResNet\_SelfA}: Local Self-Attention with ResNet
%   \item \textbf{MHA}: Multi-Head Attention
%   \item \textbf{FCN\_MHA}: Multi-Head Attention with FCN
%   \item \textbf{ResNet\_MHA}: Multi-Head Attention with ResNet
% \end{itemize}


% \subsection{Single-Step Models}

% The multi-step models extracts the features from the previous three sequences to predict the category of the final one. On the contrary, to evaluate the usefulness of patterns within single sequences, another set of neural-networks are built as part of this research. These models are designed to receive single sequences per batch and are 
% expected to learn patterns within the single sequence to help decide correct category of the sequence. This group of models are categorised as single-step models.

% Each sequence of a time-series can show patterns within itself. For example, in the case of the EEG time-series, three sequences may show that the driver is continuously in a state of distraction, but in the last sequence, while the first half of the sequence may continue distraction trends, the second half may start revealing trends of increasing driver concentration. The single-step models are designed to evaluate the performance on detecting these changes within single sequences.

% The single-step models are implemented with Multi-Head Attention layers as the attention mechanism, and FCN or ResNet as the classifier. The MHA strategy is selected because of its ability to focus on various positions of a sequence using parallel attention 'heads'. Each of these heads apply the self-attention strategy to different positions within the single sequence to extract the patterns. As discussed before, when MHA is combined with FCN and ResNet, the deep learning layers extract the features of the sequence and the attention layer simply adds a contextual vector. The architecture for this group of models is similar to the multi-step models excluding the Time-Distributed layer. 

% The single-step models implemented in this study are as follows:

% \begin{itemize}[leftmargin=*]
%   \setlength\itemsep{0.2em}
%   \item \textbf{LSA}: Luong’s Single-step Attention
%   \item \textbf{MHSA}: Multi-Head Single-step Attention
%   \item \textbf{FCN\_MHSA}: Multi-Head Single-step Attention with FCN
%   \item \textbf{ResNet\_MHSA}: Multi-Head Single-step Attention with ResNet
% \end{itemize}

% \section{Experiments}

% \subsection{Experimental Setup}

% The weakly labelled time-series used in this study are Emotiv266 and EmotivRaw, supplied by the bioinformatics company Emotiv \cite{noauthor_undated-be}. The Emotiv dataset are collections of EEG brain signals data, captured using an Emotiv headset, from participants who undertook a 40 minute driving simulation and performed various tasks while driving.

% EmotivRaw captures 14 individual EEG time-series in parallel, at a frequency of 128Hz (illustrated in Figure 1). As the participants perform various activities during driving, their brain activity alters and these are recorded in the EEG time-series. Thanks to Joseph Carl \cw{(REFERENCE)}, EmotivRaw has been spectrally transformed (using Fast-Fourier transformation \cite{Oberst2007-dh}) and the metrics for each EEG channel were aggregated to allow additional parameters to be generated. In total, 266 parameters are created and combined to form Emotiv266. 

% \subsubsection{Data Preparation}

% EmotivRaw and Emotiv266 are long lengths of multivariate time-series. To allow this data to be accepted by deep-learning models as sequences, the long time-series was segmented into equally-sized 'sequences', as shown in Figure 7.

% \begin{figure}[h]
% \centering
% \includegraphics[width=6cm]{.images/segmentation.png}
% \caption{Sequence segmentation}
% \end{figure}

% For Emotiv266, these segmented sequences are of dimensions 266 by 40, which refers to 266 parallel time-series with 40 samples in length. As Emotiv266 was captured at 4Hz, this sequence length represents approximately three sequences per second, which is a suitable simulation of a real-time stream. Each sequence is assigned with the majority label (category) of the samples, such as 0 or 1 corresponding to driving states of distracted or focused respectively.

% This study experiments with two sets of data, one with collections of four sequences per batch to be consumed by the multi-step models, and the other with just one, to be consumed by the single-step models. For the multi-step models, the four sequences together represent a window-length of 160, designed such that attention can extract context from the first 120 samples (first three sequences) to classify the final group of 40 samples (the last sequence). 

% To allow minimal data and context loss, the sequences are extracted as a sliding window with 50\% overall. This is represented by a 'stride' value, which is selected as 20 (half of sequence length).

% \subsubsection{Window Enhancements}

% While extracting sequences of size 40 and 160, each label within these sequences are compared. If the window had too many label variations (which is unlikely in Emotiv), the windows are discarded. If there are two different labels across the sequence (which is mostly the case), the sequence is split into two and filled with very small noise values to keep window sizes consistent to 40 or 160, such that each sequence now has consistent labels. This eliminates any negative impact in TSC caused by the time-series segmentation.

% \subsubsection{Up-sampling}

% Since data for distracted driving is difficult to capture, the Emotiv dataset are highly imbalanced with much more focused driving data. The number of driving to distracted sequences is 3828 to 2032 in Emotiv266, which is too imbalanced and negatively impacts the training by neural-networks. Therefore, to minimise this effect, the data is ‘up-sampled’ in its preparation phase.

% A python library ‘imblearn’ \cite{noauthor_undated-dl} is used to repeatedly duplicate random records from the minority group (distracted category). This equalises the number of records for each label and provides a fair learning opportunity for the models.

% \subsection{Experimentation}

% In this section, the proposed attention approaches are evaluated on the benchmark datasets Emotiv266 and EmotivRaw. This section discusses the impacts of the attention models and identifies various performance benefits and drawbacks of each model for weakly-labelled time-series classification. Accuracy, Area Under the Curve (AUC) and F1 scores are used as primary metrics to evaluate each model, and these metrics are compared to the existing approaches.

% It is important to note that all the models are fitted with an ADAM optimiser \cite{Kingma2014-nu}, and categorical cross-entropy is used to determine the loss per epoch. A script (available with the code) runs each mode five times with one hundred epochs.

% The models are also configured to reduce the learning rate as the loss gradient begins to flatten. This ensures the model can reach a minimum plateau in validation loss, and therefore classify with minimum loss. The experiments are also designed to ensure empirical risk minimisation by attempting to find the model with minimum loss among the epochs.

% Table 1 outlines the average validation scores of each of the models. The models are trained on training data and the metrics in this table are evaluated on test data, which are approximately 3 to 1 of Emotiv dataset respectively.

% \input{main_results_table}

% \subsection{Analysis of Scores}

% \subsubsection{Accuracy}
% Noticeable from the summary table, most of the attention implementations perform with higher accuracies than existing deep learning models. The addition of a simple LSTM layer, to interpret sequence relevance, improved the accuracy scores of FCN by 5 per cent and ResNet by 7 per cent, which is a little higher than the accuracy by ROCKET.

% The most notable models include FCN\_SelfA, MHA and FCN\_MHA, which show significant improvements in classification accuracy. On average, one of the strongest models of this research, FCN\_SelfA, classifies approximately 13 per cent more accurately compared to the existing FCN model and over 7 per cent than FCN\_LSTM on Emotiv266. Following this, FCN\_MHA and MHA perform with over 10 per cent higher accuracies than FCN, and 4 per cent higher accuracies when compared to FCN\_LSTM. Since FCN\_SelfA is the most accurate model evaluated in this experiment, further analysis is conducted on FCN\_SelfA and presented later in this paper.

% \subsubsection{AUC}
% The AUC scores are evaluated as part of the analysis to further establish the improvement by attention strategies. AUC scores are suitable for binary classification evaluation and avoid the effect of bias in the target categories when comparing the average performance of classification algorithms \cite{Huang2005-bn}. 

% The attention models show significant improvements in AUC metrics. FCN\_MHA performs with an almost 5 per cent higher AUC score compared to the FCN model, which has the highest existing AUC score. Similarly, FCN\_SelfA shows approximately 3 per cent improvement than FCN.

% \subsubsection{F1}
% The F1 scores of each model are important in this study because the initial Emotiv data is highly imbalanced. Table 1 highlights the F1 scores by existing models reaching up to a maximum average of 54 per cent. Although FCN\_SelfA and FCN\_MHA improved the F1 score by almost 4 per cent when compared to FCN, this is not a drastic improvement considering the F1 score by ROCKET is around the same.


% However, the performance metrics of the model vary as they are provided with imbalanced data. Table 2 compares the F1 and accuracy scores by the existing FCN and ResNet, and FCN\_SelfA, before the data is up-sampled during training on Emotiv266.

% \input{upsample-results}

% For FCN and ResNet, the accuracy and F1 driving scores are significantly higher when the data is imbalanced. However, the F1 distracted score is significantly low which means that the models can accurately classify most of the driving (dominant) category, but very few of the distracted (minor) category. The overall accuracy is high due to the higher true positives where in reality, most of the distracted category classifications are incorrect.


% When the data is balanced, the number of accurate distracted classifications improve, hence the distracted F1 scores rise significantly. Now that FCN and ResNet are falsely classifying for both categories, the overall accuracy falls.

% However, the metrics of FCN\_SelfA show that the effect of up-sampling has a minor effect on both the accuracy and F1 scores for driving. Moreover, the difference between the distracted F1 scores before and after up-sampling is much smaller than that of FCN and ResNet. This is because the attention strategy assists the FCN model to use the context information to make better decisions of the minor category as expected. Hence, the attention layer helps FCN to preserve the accuracy level even when the input data is imbalanced.


% \subsubsection{Effect of Overfitting}

% The bar chart shows the training, validation and test accuracies in one of the evaluations of the models on the same Emotiv266 time-series. Noticeable at first glance, almost all the models have a much higher training accuracy than test accuracy, which explains that the models are largely overfitting the training data.

% The reason for this behaviour in FCN and ResNet is due to the complex architectures of the neural network models. When these models are training on a weakly labelled dataset, they learn the noise and redundancies of the training data too accurately, which clouds their judgement of the noise as features. Thus, when the models are evaluated on test data, the models fail to identify any new patterns of noise and hence they fail to correctly extract distinctive features for binary classification.

% As expected, the attention layers significantly improve the accuracy of the models by cutting down this effect. As suggested by the results table, the attention layers can successfully identify the context of sequences, which help ResNet and FCN to identify noise and therefore, to make more informed judgements on test data.

% \begin{figure}[h]
% \centering
% \includegraphics[width=8cm]{.images/model_accuracies.png}
% \caption{Accuracy of TSC models with 100 epochs}
% \end{figure}

% \subsubsection{ResNet and FCN}

% Although the ResNet model classifies with the highest accuracy among the existing models, the results table highlights that FCN performs much better than ResNet when combined with attention layers. It suggests that the sequence relevance information contained within the feature-maps of single convolution blocks (FCN architecture) is much better interpreted by attention layers than from the feature-maps of three convoluted models (ResNet architecture). Since the architecture of ResNet is more complex, the model overfits the training data including the noise and redundancies much more than FCN.

% In fact, the accuracy scores of MHA and ResNet\_MHA suggests that MHA by itself can extract sequence features and neighbouring relevance information much better than if integrated with ResNet. This establishes that complex ResNet architecture negatively impacts the performance of the attention layers.

% \subsubsection{LATTN and BATTN}

% The performance of FCN\_LATTN and ResNet\_BATTN models show slight improvements compared to existing models, however, this enhancement is not enough to consider the use of the attention strategies by Luong et. al. or Bahdanau et. al. to improve classification accuracy. The models are considering sequence relevance information, but the simpler architecture of the models cannot retrieve enough correct context among the noise and redundancies, compared to Self-Attention or MHA models. The more complex encoders and decoders of Self-attention or MHA provide them powerful computational support to 'attend’ more areas within the previous sequences, and therefore allow higher pattern matching, which is not possible with the architectures by Luong et. al or Bahdanau et. al.

% Moreover, because of their simpler architecture, the models were evaluated on longer epochs (300 epochs) with the expectation that their performance may improve on further training. Unfortunately, the performance metrics did not improve on longer training periods and the loss graph for these evaluations are presented later.


% \subsubsection{Single-step Models}

% When evaluated on Emotiv dataset, the single-step models did not demonstrate exceptionally high accuracies. It highlights that the context of various positions within the single sequence is not enough to eliminate the effect of noise or redundancies in the case of Emotiv time-series. Therefore, the attention models require a larger window for trend analysis to fully understand the effect of noise, and so the multi-step models are performing more accurately. 

% However, these performance metrics do not disqualify the single-step models from weakly labelled TSC. Intuitively, the models will prove very useful when sequences of time-series are of high lengths and have a higher repetitive pattern within the sequences. For the case of Emotiv266 or EmotivRaw, each sequence block is not exceptionally long to allow such context analysis and hence, the single-step models show insignificant improvements compared to the existing models.

% \subsubsection{Validation Loss}

% The loss graphs illustrate how the models perform on Emotiv266 data in terms of the loss metric. The measure of loss identifies the rate of incorrect classifications by the model, and for most of the models in this research, the training loss rate shows an exponential decrease whereas the validation loss rates fluctuate and mostly, rise.

% The reason for this behaviour is once again because the models are overfitting the training data. The complex architectures help the models become over-confident during training and thus, interpret and classify validation data less accurately. For this reason, false predictions are heavily penalised by significantly increasing in validation loss but correct predictions decrease the loss insignificantly \cite{Salman2019-at}. This explains how the self-attention and MHA models are performing with higher accuracy but also with higher loss metrics.

% On the contrary, although LATTN and BATTN models have insignificant accuracy improvements, they produce a better loss pattern. This type of performance generally suggests that the models are underfitting the training data, and in the case of LATTN and BATTN, the simpler architecture of attention is responsible for this behaviour. An underfit by the attention layers mean that the attention layer is not extracting enough contextual information to have any significant effect on the performance of the model.

% \subsubsection{Global vs. Local Self-Attention}

% Both global and localised self-attention models are evaluated against the same training and validation data, and as expected, localised self-attention performed 4 per cent more accurately than global self-attention on average. This is because the model understands the noise and data redundancy trends better when it focuses on each of the three previous sequences individually, rather than a general soft-focus across the three previous sequences together. A bar chart showing detailed accuracy results for this comparison is provided in the Annex.

% \subsubsection{Additive vs. Multiplicative Self-Attention}

% When both additive and multiplicative Self-Attention with FCN are evaluated on the same data, the additive self-attention performs much better than multiplicative, with an average 5 per cent higher accuracy on on Emotiv266. During this comparison, both the models are running with localised self-attention. Bar chart showing detailed accuracy results for this comparison is provided in the Annex.

% The reason for this difference in performance is the previously discussed FFN layer, which is present in additive self-attention models but replaced by a softmax layer in the multiplicative strategy. The extra FFN layer helps the additive model interpret the encoder keys with larger dimensions. In the case of Emotiv data, the extra noise and data redundancies add additional features to learn. This adds complexity which causes the dimensions of vectors Q, K and V, generated by the encoders, to become large. The FFN layer helps compensate for this, whereas the softmax layer on the dot-product strategy cannot perform well enough. This gives additive self-attention an edge over the multiplicative model.

% \subsubsection{Normalising data}
% \input{normalisation_results}

% Table 3 shows the average outcomes when the models are evaluated on time-series with:
% \begin{itemize}[leftmargin=*]
%   \setlength\itemsep{0.1em}
%   \item No normalisation
%   \item Only normalisation during sub-sequence extraction
%   \item Only normalisation during series extraction
%   \item Both normalisation as above
% \end{itemize}

% While it is a standard practice to normalise time-series for TSC using deep-learning, the performance of the models without the two type of normalisation applied in this study, is evaluated to further reinforce the TSC improvements using attention. The outcomes in Table 3 highlights the improved performance using attention by both Self-Attention and Multi-Head Attention models.


% \section{Conclusion}
% From the experiments on the real-world Emotiv dataset, it can be concluded that the attention strategy improves the performance of existing state-of-the-art TSC algorithms on weakly-labelled time-series. To eliminate the effect of weak-labelled time-series from the real-world setting, the extraction and interpretation of sequence context information help supervised neural networks to improve their performance of sequence classification. In particular, the performance of Self-Attention with FCN (with additive function in localised context) and Multi-Head Attention with FCN displays the most dramatic improvements, and can therefore be concluded as the top models of this research.

% The set of models developed as part of this research can complement any further studies for real-time TSC.
% %\end{document}  % This is where a 'short' article might terminate


% % %ACKNOWLEDGEMENTS are optional
% % \section{Acknowledgements}
% % This section is optional; it is a location for you
% % to acknowledge grants, funding, editing assistance and
% % what have you.  In the present case, for example, the
% % authors would like to thank Gerald Murray of ACM for
% % his help in codifying this \textit{Author's Guide}
% % and the \textbf{.cls} and \textbf{.tex} files that it describes.

% %
% % The following two commands are all you need in the
% % initial runs of your .tex file to
% % produce the bibliography for the citations in your paper.
% \bibliographystyle{abbrv}
% \bibliography{sigproc}  % sigproc.bib is the name of the Bibliography in this case
% % You must have a proper ".bib" file
% %  and remember to run:
% % latex bibtex latex latex
% % to resolve all references
% %
% % ACM needs 'a single self-contained file'!
% %
% %APPENDICES are optional
% % SIGKDD: balancing columns messes up the footers: Sunita Sarawagi, Jan 2000.
% % \balancecolumns
% \appendix

% \section{Self-Attention Comparisons}

% \begin{figure}[h]
% \centering
% \includegraphics[width=7cm]{.images/selfa_FCN_vs_selfa_FCN_Global.png}
% \caption{Accuracy of Global vs. Local SelfA}
% \end{figure}


% \begin{figure}[h]
% \centering
% \includegraphics[width=7cm]{.images/additive_vs_multiplicative_sefl_Attn.png}
% \caption{Accuracy of Additive vs. Multiplicative SelfA}
% \end{figure}

% \section{Validation Loss Graphs}
% \cw{CW: If we are not using them, then we should remove these graphs from the appendix and paper}
% \begin{figure}[h]
% \centering
% \includegraphics[width=6cm]{.images/epochs_loss_fcn_lstm.png}
% \caption{Epoch loss of FCN\_LSTM}
% \end{figure}

% \begin{figure}[h]
% \centering
% \includegraphics[width=6cm]{.images/epochs_loss_ResNet_LSTM.png}
% \caption{Epoch loss of ResNet\_LSTM}
% \end{figure}

% \begin{figure}[h]
% \centering
% \includegraphics[width=6cm]{.images/epochs_loss_SelfA_FCN.png}
% \caption{Epoch loss of FCN\_SelfA}
% \end{figure}

% \begin{figure}[h]
% \centering
% \includegraphics[width=6cm]{.images/epochs_loss_MHA_FCN.png}
% \caption{Epoch loss of FCN\_MHA}
% \end{figure}

% \begin{figure}[h]
% \centering
% \includegraphics[width=6cm]{.images/epochs_loss_LATTN_FCN.png}
% \caption{Epoch loss of FCN\_LATTN}
% \end{figure}

% \begin{figure}[h]
% \centering
% \includegraphics[width=6cm]{.images/epochs_loss_BATTN_FCN.png}
% \caption{Epoch loss of FCN\_BATTN}
% \end{figure}




% % %Appendix A
% % \section{Headings in Appendices}
% % The rules about hierarchical headings discussed above for
% % the body of the article are different in the appendices.
% % In the \textbf{appendix} environment, the command
% % \textbf{section} is used to
% % indicate the start of each Appendix, with alphabetic order
% % designation (i.e. the first is A, the second B, etc.) and
% % a title (if you include one).  So, if you need
% % hierarchical structure
% % \textit{within} an Appendix, start with \textbf{subsection} as the
% % highest level. Here is an outline of the body of this
% % document in Appendix-appropriate form:
% % \subsection{Introduction}
% % \subsection{The Body of the Paper}
% % \subsubsection{Type Changes and Special Characters}
% % \subsubsection{Math Equations}
% % \paragraph{Inline (In-text) Equations}
% % \paragraph{Display Equations}
% % \subsubsection{Citations}
% % \subsubsection{Tables}
% % \subsubsection{Figures}
% % \subsubsection{Theorem-like Constructs}
% % \subsubsection*{A Caveat for the \TeX\ Expert}
% % \subsection{Conclusions}
% % \subsection{Acknowledgements}
% % \subsection{Additional Authors}
% % This section is inserted by \LaTeX; you do not insert it.
% % You just add the names and information in the
% % \texttt{{\char'134}additionalauthors} command at the start
% % of the document.
% % \subsection{References}
% % Generated by bibtex from your ~.bib file.  Run latex,
% % then bibtex, then latex twice (to resolve references)
% % to create the ~.bbl file.  Insert that ~.bbl file into
% % the .tex source file and comment out
% % the command \texttt{{\char'134}thebibliography}.
% % % This next section command marks the start of
% % % Appendix B, and does not continue the present hierarchy
% % \section{More Help for the Hardy}
% % The acmproc-sp document class file itself is chock-full of succinct
% % and helpful comments.  If you consider yourself a moderately
% % experienced to expert user of \LaTeX, you may find reading
% % it useful but please remember not to change it.

% % That's all folks!


% \end{document}


==> backup/backup_main2.tex <==
% % It is an example file showing how to use the 'sigkddExp.cls' 
% % LaTeX2e document class file for submissions to sigkdd explorations.
% % It is an example which *does* use the .bib file (from which the .bbl file
% % is produced).
% % REMEMBER HOWEVER: After having produced the .bbl file,
% % and prior to final submission,
% % you need to 'insert'  your .bbl file into your source .tex file so as to provide
% % ONE 'self-contained' source file.
% %
% % Questions regarding SIGS should be sent to
% % Adrienne Griscti ---> griscti@acm.org
% %
% % Questions/suggestions regarding the guidelines, .tex and .cls files, etc. to
% % Gerald Murray ---> murray@acm.org
% %

% \documentclass{sigkddExp}

% \input{packages.tex}

% \graphicspath{ {./images/} }

% \def\cw#1{\textcolor{blue}{#1}}

% \begin{document}
% %
% % --- Author Metadata here ---
% % -- Can be completely blank or contain 'commented' information like this...
% \conferenceinfo{ACM SIGKDD}{Singapore} % If you happen to know the conference location etc.
% %\CopyrightYear{2001} % Allows a non-default  copyright year  to be 'entered' - IF NEED BE.
% %\crdata{0-12345-67-8/90/01}  % Allows non-default copyright data to be 'entered' - IF NEED BE.
% % --- End of author Metadata ---

% \title{Classification of multivariate weakly-labelled time-series with attention}
% %\subtitle{[Extended Abstract]
% % You need the command \numberofauthors to handle the "boxing"
% % and alignment of the authors under the title, and to add
% % a section for authors number 4 through n.
% %
% % Up to the first three authors are aligned under the title;
% % use the \alignauthor commands below to handle those names
% % and affiliations. Add names, affiliations, addresses for
% % additional authors as the argument to \additionalauthors;
% % these will be set for you without further effort on your
% % part as the last section in the body of your article BEFORE
% % References or any Appendices.

% \numberofauthors{1}
% %
% % You can go ahead and credit authors number 4+ here;
% % their names will appear in a section called
% % "Additional Authors" just before the Appendices
% % (if there are any) or Bibliography (if there
% % aren't)

% % Put no more than the first THREE authors in the \author command
% %%You are free to format the authors in alternate ways if you have more 
% %%than three authors.

% \author{
% %
% % The command \alignauthor (no curly braces needed) should
% % precede each author name, affiliation/snail-mail address and
% % e-mail address. Additionally, tag each line of
% % affiliation/address with \affaddr, and tag the
% %% e-mail address with \email.
% \alignauthor Surayez Rahman \\
%        \affaddr{Faculty of Information Technology}\\
%        \affaddr{Monash University, Clayton Campus}\\
%        \affaddr{Melbourne, Australia}\\
%        \email{srah0001@student.monash.edu}
% \alignauthor Chang Wei Tan\\
%        \affaddr{Faculty of Information Technology}\\
%        \affaddr{Monash University, Clayton Campus}\\
%        \affaddr{Melbourne, Australia}\\
%        \email{chang.tan@monash.edu}
% % \alignauthor Mahsa Salehi\\
% %       \affaddr{Faculty of Information Technology}\\
% %       \affaddr{Monash University, Clayton Campus}\\
% %       \affaddr{Melbourne, Australia}\\
% %       \email{mahsa.salehi@monash.edu}
% }

% \date{06 November 2020}

% \maketitle
% \begin{abstract}
% In this research, a gap is identified in the field of real-time time-series classification (TSC) on multivariate weakly-labelled time-series. As it will be shown in the paper, weakly labelled time-series are subsequences containing noise and significant redundancies, and 
% low classification accuracy is observed in this study when existing state-of-the-art TSC models are evaluated on such data. In response to this gap, this paper proposes an approach of exploiting context relevance of subsequences from previous subsequences to improve classification accuracy. To achieve this, state-of-the-art Attention algorithms are experimented in combination with the top CNN models for TSC (FCN and ResNet), in an encoder-decoder architecture. Attention is a popular strategy with exceptional performance in modern sequence-to-sequence analysis, and this paper shows how attention algorithms can be used for improved TSC. To evaluate this improvement, multivariate EEG time-series are obtained using commercial Emotiv headsets from participants performing various activities while driving. These time-series are segmented into subsequences and labelled to allow supervised TSC.

% \end{abstract}




% \section{Introduction}
% Time-series classification \cw{(TSC)} is one of the most well-researched areas of modern computer science \cite{Bagnall2017-xw}. 
% \cw{With the increase in time-series data, accurate real-time TSC has become more important than ever.}
% % With the rise in time-series data analysis, real-time time-series classification is a very important concept in the current world scenario. 
% Despite the huge progress in \cw{TSC} over the last decade \cite{Bagnall2017-xw}, most of these work make assumptions that are unrealistic in the real-world setting. 
% This includes the assumption that the patterns (subsequences) that exist in the time-series are of fixed equal lengths and are always correctly labelled \cite{Hu2016-go}. 
% However, in the real-world settings, these patterns can be of unequal length, the class label of the pattern may contain errors and may only correspond to a general section of the data.
% More importantly, the class labels are typically highly imbalanced.
% % and filled with noise or other redundancies, as will be shown in this paper.
% % To illustrate an example

% \cw{For example, detecting distracted driving using Electroencephalography (EEG) signal is a challenging task that violates the unrealistic assumptions required by most TSC algorithms.
% Figure \ref{fig:eeg} shows an EEG signal}
% obtained from a participant during driving using \cw{the} Emotiv Epoc+ EEG headset \footnote{\url{https://www.emotiv.com/epoc/}}. 
% The 14\cw{-channel EEG signal can be interpreted as a time-series with 14 dimensions.
% A time-series analysis algorithm can be applied to analyse these brain waves of the driver and detect the state of the driver to be either focused or distracted.} 
% % time-series here are captured simultaneously and each of them represents a single channel of EEG brain signals.
% \cw{The different colors, as indicated in the legend, represent the different activities performed by the driver during driving.
% These activities are weakly labelled because it is challenging to correctly label the driver's transition from driving to using an iPad and vice versa.
% Besides, these subsequences may also contain noise or redundant patterns that are not related to the activity that driver is performing at that point in time.
% In fact, these redundant patterns may occur in different activity patterns, which makes it challenging to differentiate the different activities.}
% % \cite{noauthor_undated-rv}.
% % , where the x-axis represents time, the y-axis signifies fluctuations in brain signals. 
% % Each sequence is coloured to represent different activities during driving as shown in the legend.
% % When collected raw, the data are not labelled as such and there are no distinct points to when the driver transitions from driving to using an iPad. The only annotation given for this data is that it represents brain signals of a driver who is generally focused. 
% % \cw{Typically}, in such \emph{weakly labelled} time-series, each \cw{subsequence tend to be} very similar to the other \cw{subsequences, even when they have different labels. 
% % This makes it extremely challenging to differentiate the subsequences of different labels.}
% % due to the overlay of recorded noise and each sequence are of varying lengths. 
% % Typically such time-series are highly imbalanced such that they contain much more driving data than distracted data.
% % Moreover, such multivariate data can only make sense if these parallel time-series are analysed together and therefore, it elevates the difficulty for algorithms to consume and build an understanding of the data.
% \cw{Moreover, most real-world time-series dataset are highly imbalanced where they contain more of the ``normal'' label.
% In this example, there are more driving labels than distracted labels, thus making the task of predicting a distracted activity extremely challenging.}
% % Typically such time-series are highly imbalanced such that they contain much more driving data than distracted data.
% % Moreover, such multivariate data can only make sense if these parallel time-series are analysed together and therefore, it elevates the difficulty for algorithms to consume and build an understanding of the data.

% \begin{figure}[t]
% % \centering
% \includegraphics[width=\linewidth]{.images/Emotiv14.pdf}
% \caption{Example of a weakly labelled EEG data}
% \label{fig:eeg}
% \end{figure}

% \cw{Quite simply, current state-of-the-art TSC algorithms are not capable of handling weakly labelled time-series data.}
% % For time-series classification, Fully Convolutional Network (FCN) and Residual Network (ResNet) are two state-of-the-art deep learning algorithms \cite{Ismail_Fawaz2019-tc}, but unfortunately, when these models were evaluated in this research, they demonstrated poor accuracies in classifying multivariate weakly-labelled time-series. 
% It makes sense because these models were mainly designed
% % to extract and interpret features from 
% \cw{for univariate TSC.} 
% % individual sequences to classify their category. 
% While this strategy works well for noise-free time-series with proper
% % annotations
% \cw{labeling}, it fails to extract discriminative features from weakly-labelled time-series as it cannot distinguish between noise and useful data, especially when the class labels are highly imbalanced.

% This research
% % identifies a requirement
% \cw{aims} to develop 
% % generalised supervised-neural-network models 
% \cw{models} that can accurately classify multivariate weakly-labelled time-series in real-time. 
% The approach explores the use of ``attention'' strategies \cite{Bahdanau2014-eh} to extract the contextual relevance of sequences, 
% % using which noise and redundancies from data can be eliminated during classifications.
% \cw{while minimising the effect of noise and redundancies.}
% The intuition behind this is the chronological order of time-series, such that under realistic conditions, they follow certain chronological trends. 
% For example, \cw{for the task of predicting distracted driving, the EEG data}
% % in the EEG time-series, the data 
% will typically show a driver who is distracted at one moment has a higher probability of being distracted in the next moment or show gradual changes, rather than a sudden spike in concentration.
% Therefore, this research studies a set of deep learning models that can classify each subsequence of the time-series and understand sequence correlations using attention.
% % to resolve noise. The attention models are adapted from original designs in the field of NLP and are implemented within existing state-of-the-art deep learning models to classify weakly labelled multivariate in real-time with better performance than existing models.

% % \cw{This paper is organised as follows.... Section ... describe XXXX...}
% This paper is organised as follows. Section \ref{sec:background} discusses some background information and related work in state-of-the-art TSC algorithms and introduces existing attention strategies. Section \ref{sec:methodology} highlights the improvements made using an encoder-decoder architecture to implement the idea of context relevance. It also describes the use of LSTM and attention strategies. Finally, sections \ref{sec:experimentation} and \ref{sec:performancediscussion} describe the experimental setup with the weakly labelled time-series evaluated in this research, followed by the improved results discussion obtained as a result of this study.

% % This paper is organised in a structure where:
% % 1. \textbf{Background and Related Work} section discusses the state-of-the-art TSC algorithms and their performance gap on weakly labelled data. It also introduces existing attention strategies which display exceptional performance in the field of sequence-to-sequence analysis.


% % 2. \textbf{Methodology} highlights the attempted improvements on existing TSC algorithms using an encoder-decoder architecture to implement the idea of context relevance. It describes the use of LSTM and latest attention strategies.


% % 3. \textbf{Experimentation} section describes the experimental setup and the weakly labelled time-series evaluated in this research followed by the improved results obtained from all the models, and


% % 4. \textbf{Performance Discussion} which pin-points the exact improvements in TSC as a result of this study.

% \section{Background and Related Work}
% \label{sec:background}
% The field of TSC has advanced significantly in the last decade, with each algorithm significantly more accurate than its predecessors.
% This section outlines the strength and limitations of some of the existing state-of-the-art TSC algorithms \cw{used in this research} and some of the popular attention strategies available till date.

% \subsection{State-of-the-art TSC Algorithms}
% \label{subsec:sota tsc}
% % In 2020, 
% \cw{Recently,} Dempster et. al. \cite{Dempster2020-ck} proposed ROCKET, a \cw{TSC classifier that achieves state-of-the-art performances with a fraction of time of existing state-of-the-art methods.
% ROCKET extract features from a time-series using a large number of random convolutional kernels. 
% These kernels have random length, weights, bias, dilation, and padding, and when applied to a time-series produce a feature map.
% Then the maximum value and the proportion of positive values are computed from each feature map, producing two real-valued numbers as features per kernel.
% With the default 10,000 kernels, ROCKET produces 20,000 features.
% These features are then used to train a ridge regression classifier.
% ROCKET was found to be the most accurate TSC classifier compared with other state-of-the-art algorithms such as HIVE-COTE \cite{lines2016hive}, InceptionTime \cite{fawaz2019inceptiontime} and ResNet \cite{Ismail_Fawaz2019-tc} when bench-marked on the 85 TSC dataset \cite{dau2019ucr}.}
% % feature-extraction model using random convolutional kernels for univariate TSC. ROCKET is scalable and achieves state-of-the-art performance in TSC \cite{Dempster2020-ck}.
% \cw{Although designed for univariate time-series,} it can easily be adapted for multivariate \cw{time-series} with similar performance. 
% This research applies ROCKET on weakly-labelled multivariate time-series, however as shown later,
% \cw{ROCKET does not perform well on weakly labelled time-series because it was designed using clean, well-labelled time-series dataset \cite{dau2019ucr}.}
% % the performance of the \cw{algorithm} is not accurate enough, particularly on time-series containing large quantities of noise and redundancies. 
% % This was expected as ROCKET was not designed to classify weakly labelled time-series. 
% In fact, none of the state-of-the-art TSC algorithms are designed to classify weakly labelled time-series.
% % in real-time.

% % Previously in 2019, 
% Ismail et. al. \cite{Ismail_Fawaz2019-tc}
% % evaluated
% \cw{reviewed a few} 
% % state-of-the-art 
% deep-learning models \cw{for TSC}.
% \cw{They found two models that achieve state of the art performances,} Fully \cw{Convolutional} Network (FCN) and Residual Network (ResNet).
% \cw{ResNet was ranked as the most accurate univariate TSC deep learning model bench-marked on 85 univariate TSC dataset \cite{dau2019ucr}. 
% It is a convolutional neural network (CNN) that consists of three residual blocks with three convolutional layers in each block, followed by a global average pooling (GAP) layer and a softmax layer for classification.} In some time-series, the changes in data are very small, which means their learning gradient is extremely small. \cw{On the other hand, when bench-marked on 12 multivariate TSC dataset, FCN is the most accurate multivariate TSC deep learning model although it is not significantly different from ResNet \cite{Ismail_Fawaz2019-tc}. 
% } 
% % for TSC. 
% % FCN and ResNet are both deep-learning convolutional neural-networks (CNNs), that learn features from time-series by generating a set of feature-maps.
% FCN 
% % contains
% \cw{consists of} three \cw{1D} convolutional blocks \cw{with batch normalisation and ReLU activation function to learn features from the time series.} 
% % These blocks create and update feature-maps which are, in fact, representations of the features learnt by the model. 
% % A subsequence 
% \cw{Then, a GAP} layer\cw{, applied to the last convolutional block summarises the features which is then passed to a softmax classifier for classification.} 
% % takes the average pooling of the features, on which a final softmax function generates a probability distribution that is used to determine the label of input data.

% % Similarly, ResNet contains nine convolutional blocks, but it includes residual connections which provide the additional ability to take ’shortcuts’. These shortcuts escalate the model to learn and classify very quickly and help the model reduce the vanishing gradient effect\cite{Hochreiter1998-uf}. In some time-series, the changes in data are very small, which means their learning gradient is extremely small. With the help of residual connections, ResNet eliminates these inaccuracies. The rest of the structure of ResNet is identical to FCN.

% % This is important in this study because it prevents inaccurate training on weakly labelled time-series that have tiny variations. Finally, ResNet has a GAP layer at the very end that enables the model to generally work well across a variety of time-series data.

% % ResNet is a special model with residual connections that help it reduce any vanishing gradient effect 
% % \cw{CW: describe the models a bit more in details like what I did for Rocket.}



% % The architecture for these two models are important to this study and are discussed below in detail.
% % \cw{\subsubsection{Fully Convolutional Network (FCN)}}

% % \cw{FCN model has three convolutional blocks and a final Global Averaging Pool (GAP) layer. The first convolution block creates a set of feature-maps and then passes it on to the next block. Each feature map is a representation of various features learnt by the model for a sequence. The next two blocks further improve and update these feature-maps, and pass them to the GAP layer. The GAP layer takes the average pooling of the features, on which a softmax function is applied in the final dense layer to determine the class of the sequence.}

% % \cw{\subsubsection{Residual Network (ResNet)}}

% % \cw{ResNet is designed with nine convolutional neural blocks, which work similar to the FCN model, and includes an additional ability to take ’shortcuts’ using residual connections. These shortcuts escalate the model to learn and classify very quickly and help the model reduce the vanishing gradient effect. In some time-series, the changes in data are very small, which means their learning gradient is extremely small. While a general neural model learns these changes negligibly, with the help of residual connections, ResNet can overcome these inaccuracies. This is important in this study because it prevents inaccurate training on weakly labelled time-series that have tiny variations. Finally, ResNet has a GAP layer at the very end that enables the model to generally work well across a variety of time-series data.}

% % While these CNN models can be used to classify multivariate time-series, 
% % % in real-time, 
% % their design focused on classifying clean and processed time-series, unlike in a real-world setting. 
% % \cw{Similar to ROCKET, they do not perform well on weakly labelled data, as will be shown in Section XX.}
% % As this research evaluated their performance on weakly labelled data, the metrics are not exceptional, as will be shown later in the paper. 

% % \cw{CW: I will add on some more related work here. There are a few other algorithms that should be described here as well.}

% % In 2019, 
% Perslev et. al. \cite{Perslev2019-db} 
% % introduced
% \cw{proposed U-Time, a segmentation algorithm}
% % an advanced segmentation algorithm called U-Time, 
% which uses a feed-forward network (FFN) with convolutional encoders and decoders to segment subsequences of long time-series. 
% U-Time \cw{was designed for segmentation and} demonstrated high segmentation accuracy on a range of multivariate weakly labelled time-series such as real-life sleep-staging \cw{EEG} time-series. 
% \cw{In this research, we are interested in the classification of weakly labelled data. Hence U-Time is not being evaluated in this work and will be considered as future work.}
% % The model can be expected to classify multivariate weakly labelled time-series successfully, however, due to the nature of feed-forward networks (FFNs), the complete input time-series must be provided to the model before it can segment each subsequence of the time-series. Using this algorithm is a drawback for real-time classification, where data need to be streamed continuously and the model would need to analyse new prevailing subsequences. For real-time analysis, U-Time would become computationally expensive and hence, it is not the most appropriate model out of the box. However, U-time can be explored in future to apply the intuition for real-time time-series classification.

% % ROCKET, FCN, \cw{and} ResNet 
% % % U-Time
% % are 
% % % among the most recent and advanced
% % state-of-the-art multivariate TSC algorithms that are also scalable.
% % but none are designed to interpret weakly labelled data correctly in real-time. 
% \cw{All of these state-of-the-art algorithms have shown superior performance on a set of benchmark dataset \cite{dau2019ucr}.
% Most of these dataset are not realistic, i.e. they are properly labelled, equal in length and do not suffer from class imbalanced.
% Hence these state-of-the-art algorithms are not capable of handling weakly labelled dataset with unequal length and highly imbalanced, such as the task of predicting distracted driving using EEG signal, as shown in our experiments in Section \ref{sec:experimentation}.}
% Therefore, this research identifies the lack of a 
% % proper
% \cw{suitable algorithms} 
% % model
% to classify multivariate weakly-labelled time-series 
% % in real-time 
% with high accuracy.

% Among these existing state-of-the-art models, this research focuses on \cw{improving} FCN and ResNet because their neural network architecture allows them to be upgraded. 
% \cw{More specifically, this paper explores various attention strategies to handle weakly labelled data.}
% % If these models can remove noise and redundancies from weakly labelled data, they will be able to drastically improve their performance. 
% % One of the ways of doing this efficiently is to learn the contextual relevance of the subsequences.
% % Expanding on this idea, this research introduces attention strategies, to allow deep learning models to get a comprehensive understanding of the context of input time-series.


% \subsection{Attention}

% The attention concept was initially proposed in 2015 by Bahdanau et. al. \cite{Bahdanau2014-eh} to utilise the contextual information in sequence-to-sequence (Seq-2-Seq) problems such as natural language processing (NLP) \cite{Bahdanau2014-eh}. 
% Seq-2-Seq models are neural networks that \cw{take in a sequence of data as input} and output \cw{another sequence, such as language translation.} 
% % continuous sequences of data. 
% These models typically \cw{consists of an encoder and a decoder.}
% % encoder-decoder architectures, where the encoder consumes the complete input sequences before decoding the output sequence. 
% \cw{The encoder tries to summarise the input sequence into a concise feature vector while the decoder maps the feature vector to an output sequence.
% Using the example of language translation, the input can be an English sentence and the output can be a French sentence.}
% When input sequences are long, generating the contextual information becomes a bottleneck. 
% To prevent this problem, attention strategy was introduced to decouple the encoders and decoders, and allow long sentences to be translated accurately using alignment functions.
% % \cw{CW: should you mention that attention assigns weights to the sequences? I am doing that later in methodology}

% \subsubsection{Attention by Luong and Bahdanau et. al.}
% Since the introduction of attention, several other designs were introduced by a number of subsequent papers, mostly focused on language translation.
% % \cw{CW: do you mean language translation here?}. 
% In 2015, Luong et. al \cite{Luong2015-xr} proposed an attention model in an \cw{Long Short-Term Memory} (LSTM) encoder-decoder architecture.
% Their model 
% % \cw{CW: which model is this?} 
% was based on the intuition to keep track of all the words in a sentence so that the relevance of each word to the current word can be used to make better translation decisions. 
% Luongs' attention 
% % \cw{CW: Which attention is this?} 
% was an improvement to the previous strategy by  Bahdanau et. al. \cite{Bahdanau2014-eh}, because it uses multiple calculations to derive the context. However, the benefit of the model by Bahdanau et. al. \cite{Bahdanau2014-eh} was that it extracted bi-directional sequence context.

% \subsubsection{Self-Attention and Multi-Head Attention}
% Later in 2017, a state-of-the-art attention model, known as Multi-Head Attention, were proposed by Vaswani et. al. \cite{Vaswani2017-xw} 
% % \cw{CW: I think you can just say multi-head attention and describe it in terms of self-attention}.
% To learn the context in sequences, this model builds correlation functions using a neural network model known as Self-Attention and use a complex multi-layered encoder-decoder architecture, known as the Transformer \cite{Vaswani2017-xw}. This model can focus on multiple sections of sequences in parallel to extract context.
% % \cw{CW: what do you mean by seq-2-seq data? do you mean seq-2-seq problems?}. 


% Since the introduction of these attention models, they have been adopted in  various research across different problem domains \cite{Weng2018-fc}. In this research, some of the above-mentioned attention strategies \cw{are explored} in combination with the existing CNN TSC algorithms to demonstrate significant improvement in TSC.

% % \cw{I think you have mentioned this in the methodology (3.1), so this paragraph can be skipped.}
% % This research \cw{explores and} studies the above-mentioned set of attention strategies thoroughly.
% % \cw{More specifically, this research extends existing CNN TSC algorithms using LSTM layers and attention mechanisms}
% % to allow context of time-series subsequences to be extracted. 
% % % These algorithms are recreated within an CNN-LSTM encoder and decoder architecture, to allow context of time-series subsequences to be extracted, and in combination with existing CNN TSC models, 
% % \cw{We show that the combination of these architectures performs significantly better than existing CNN TSC models}. 
% % % the new set of models are expected to perform significantly better than existing implementations.


% \section{Methodology}
% \label{sec:methodology}

% \cw{This section outlines the approach taken in this study to improve existing TSC models on weakly labelled data.}
% % The approach taken in this study to improve TSC is explained step-by-step across the following sections.
% The first sub-section discusses the intuition behind the use of context-relevance to improve weakly labelled TSC. 
% The subsequent sub-sections illustrate the encoder-decoder architecture implemented in this research, discusses CNN with LSTM for basic context extraction and finally, explains the implementation of existing attention strategies for complex context extraction in TSC.

% % Methodology Structure:
% % 1. The idea of context relevance
% % 2. Enc-Dec architecture to allow context extraction
% % 3. LSTM attempted + slight improvement + still can be improved
% % 4. Implementing various existing attention strategies to ResNet/FCN.

% % \cw{CW: I think it is better to have this section organised in this way. Start with some motivation that FCN or typical TSC algorithms failed (point to the results section), then talk about encoder decoder structure where we use FCN-LSTM etc and finally add attention to it.}


% \subsection{Context relevance of subsequences}

% Relevance information in time-series can be described as additional context between subsequences.
% % for example, ``two previous subsequences from a same category have sections that show similar patterns as the current subsequences''. 
% % \cw{CW: maybe this is better? 
% \cw{For example, if the current subsequence has the same class as the previous two subsequences, they are likely to have similar patterns that can help to improve the TSC.}
% When the 
% % existing supervised neural-networks 
% \cw{models} incorrectly learn the 
% % distinctive 
% features from subsequences due to noise and erroneous data, these additional context can help the models identify similar sections of a subsequence with previous subsequences to correctly identify its category.
% This means \cw{that} even if the current subsequence is much longer or shorter in length, \cw{by}
% % simply 
% finding relevant sections from previously known subsequences can help the model understand the correct category of the subsequence. Therefore, it eliminates the effect of subsequence length variations in TSC.

% Similarly, if the data is imbalanced and the model does not have enough data to learn the features of the minority category, the contextual information can tip the classification decision for a subsequence towards the correct category as soon as it detects relevant sections with previous subsequences which also belong to that minority category.

% Since time-series data \cw{are ordered in time,}
% % follows \cw{a} continuous order, 
% the level of noise or redundancy is expected to show continuous changes.
% If a model can constantly keep track of the noise and redundancies by comparing the relevance of sections from previous subsequences, it can continuously learn and cancel out the effect of noise or redundancies. With this intuition, two aspects of a desired neural network can be defined; it must be supervised to firstly allow the model to learn correct features corresponding to categories and secondly, it must be able to keep track of the contextual information for every subsequence with its nearest previous ones. 

% Following this idea, this study \cw{employs an encoder-decoder structure to learn the relationship between subsequences.} 
% State-of-the-art supervised CNN TSC models- FCN and ResNet are used to learn subsequence features, and 
% % explores experiments with 
% various context-extraction approaches, involving LSTM and Attention \cw{are explored}.


% \subsection{The Encoder-Decoder architecture}
% \cw{CW: After reading this in more details, I think we should move the encoder-decoder structure with attention and this section will just focus on CNN-LSTM.}
% % When deep learning layers receive four subsequences together in a batch, they create a single set of feature-maps for the complete length of the input time-series. These feature-maps are not useful if they are directly passed to an attention layer because attention cannot segment the feature-maps for each subsequences. To prevent this, a Time-Distributed layer from the Keras library is introduced after the deep learning layers. The time-distributed layer acts as a wrapper that slices the feature-maps into four sections for each subsequence, and passes them onto an LSTM encoder. 

% % The deep-learning \cw{TSC} models, FCN and ResNet, are built with convolutional blocks. 
% % This allows them to learn distinctive features of time-series subsequences and then classify subsequences into categories based on the features. However, for these models to understand and interpret additional context relevance information between subsequences, an encoder-decoder architecture is required.

% Generally, encoder-decoder architectures are designed with LSTM encoders and LSTM decoders in seq-2-seq models \cw{put reference}. 
% However, this study has decided to use CNN encoders and LSTM decoders (a CNN-LSTM architecture). 
% This is because the CNNs \cw{have shown to achieve state of the art performances on various TSC tasks \cite{Ismail_Fawaz2019-tc}.} 
% \cw{CNNs} are 
% % required 
% \cw{used} to extract distinctive features from subsequences \cw{while LSTMs are used to learn the relationship between subsequences.}
% % and only after this, the additional context information can be made use of. 
% % Afterwards, the LSTM decoder can step through the context vector returned from context analysis algorithms to combine them back to the output from CNN.
% % To illustrate the architecture implemented in this study, 
% Figure \ref{fig:cnn-lstm} \cw{illustrates a general CNN-LSTM architecture that is used in this study, using FCN as the encoder and two LSTM layers.
% Note that the FCN layers can be replaced by any CNN layers while}
% % FCN with CNN-LSTM. 
% % In this architecture, 
% LSTM or Attention layers can be placed in between the CNN encoder and the LSTM decoder for subsequence context extraction.

% % When attention algorithms are used to extract context, they perform calculations on the feature maps of each subsequence. As the attention needs to extract information from 4 subsequences, it needs a way to retain such small blocks of data to allow it repeatedly use them for contextual analysis. This is where encoders and decoders come to the picture.

% \begin{figure*}[ht]
% \centering
% \includegraphics[width=14cm]{.images/CNN_LSTM_ENCDEC.pdf}
% \caption{\cw{A general} CNN-LSTM architecture using \cw{FCN as the CNN encoder, where $N$ is the number of subsequences.} \cw{CW: I think this image is incorrect. Your input should be 40 x L x N. and the convolution layers should be 128 x L. Maybe try creating something like figure 1 of \url{https://www.cv-foundation.org/openaccess/content_cvpr_2015/papers/Donahue_Long-Term_Recurrent_Convolutional_2015_CVPR_paper.pdf}}}
% \label{fig:cnn-lstm}
% \end{figure*}

% % On a high level, the LSTM decoder steps through the CNN feature-maps and convert them into a fixed length context vector. The context extraction algorithms can now use this context vector to store the additional context. 

% % To illustrate the architecture implemented in this study, Figure 2 shows FCN with CNN-LSTM. In this architecture, LSTM or Attention layers can be placed in between the CNN encoder and the LSTM decoder for subsequence context extraction.

% This design 
% % would be
% \cw{is} applicable for both univariate and multivariate time-series. 
% As illustrated in Figure \ref{fig:cnn-lstm}, $N$ number of subsequences can be provided to this CNN-LSTM encoder-decoder.
% % to create feature-maps and extract context of each subsequence. 
% However, to prevent the likelihood of ``vanishing gradient'' \cite{Hochreiter1998-uf} in LSTM, a suitable number of subsequences need to be selected.
% \cw{CW: don't think this is the reason.}
% \cw{This study implements this design with four subsequences as it was found to be more realistic in the problem of detecting distracted driving where each subsequence corresponds to 2 or 11.75 seconds of EEG signal. CW: I think we can mention this in the experiments where the problem is introduced. In this section, we should just be more general on describing the method}
% % Therefore, this study implements this design with four subsequences per batch, so that 
% The first $N-1$ subsequences
% % three sequences can be
% \cw{are} used to extract context and when combined with the feature-maps from the CNN layers, the final subsequence in the batch can be classified \cw{more accurately}.

% % The data provided to the encoder-decoder models are 4 subsequences with 40 time-steps and 266 parameters.
% % In the case of FCN, as shown in Figure 2, the subsequences are filtered by 3 convolutional blocks with filter size of 128, 256 and 128 respectively. The idea remains the same when ResNet is used, which has an additional 6 convolutional blocks.

% % Each of these encoders encode their own feature-maps and pass them to the next layers. The attention layers process these feature-maps in their own strategies (discussed later in the paper) and concatenate their information to update the context vectors. Each of these context vectors now flow to individual LSTM decoders to be decoded into four sets of feature maps. Finally, a GAP layer averages these feature maps into a single set, and passes onto a softmax function to obtain probability distributions.

% % Now that the CNN-LSTM architecture is implemented, the context-extraction algorithms can be added to FCN and ResNet. The next few sections of this paper describe how LSTM and Attention algorithms are added for improve TSC.



% \subsection{LSTM for basic context extraction}

% % The deep-learning models, FCN and ResNet, are built with convolutional neural network (CNN) blocks, which allow them to learn distinctive features of time-series sequences and classify them into categories based on the features. Additionally, to learn the context relevance of each sequence from its previous subsequences, this research adds an LSTM layer to FCN and ResNet.
% \cw{CW: I think this section can be merged with the previous section.}
% LSTM is a popular Recurrent Neural Network (RNN). The benefit of using an RNN layer, is its 
% % additional 
% ability to ``remember from the past'' \cw{CW: add citations}. 
% LSTM has the ability to store context because it is influenced by both its given input weights and hidden-state vectors that represent context from previous inputs. 
% % In the case of this research, this capability is used to store the contextual information of the feature-maps passed from the the CNN. 

% % Moreover, LSTMs can typically accept one or more input vectors and can output one or more output vectors. 
% % In this study, this ability of LSTM is used to process multiple subsequence feature-maps simultaneously.

% Using LSTM as a context extraction layer, two of the following models are created:
% \begin{enumerate}
%   \item FCN\_LSTM 
%   \item ResNet\_LSTM
%  \end{enumerate}

% % In both these models, the CNN layers are followed by two LSTM layers and a softmax layer. Figure 2 shows the architectural dimensions in detail.

% % \begin{figure}[h]
% % \centering
% % \includegraphics[width=8cm]{.images/CNN_LSTM.png}
% % \caption{CNN-LSTM architecture}
% % \end{figure}

% % Both of these models are trained on 4 subsequences with 40 time-steps and 266 parameters. 
% \cw{Try to describe the following in a more general way in terms of N. We will talk about the 4 in the experiments section.}
% After the CNN layers encodes these into feature-maps, they are passed to the first LSTM layer in groups of 4 (one for each subsequence). 
% \cw{CW: I don't think these LSTMs creates the context vector. The context vector is created from the CNNs and the LSTM just try to decode it.}
% The LSTM extracts context and creates ``context vectors''. 
% When passed to the LSTM decoders, these context vectors are added back to the feature-maps. 
% Finally, the softmax layer normalises these updated feature-maps to a probability distribution to allow the classification of subsequences.

% Table 1, in the results section, show the improvements made with LSTM context analysis. While this approach does improve the classification performance when compared to FCN or ResNet, the performance can be further improved using more complex context relevance analysis. Expanding on the idea, the existing attention strategies are added to the encoder-decoder architecture for context extraction.


% \subsection{Attention for advanced context extraction}
% \cw{CW: Here, we should talk about how attention can improve on CNN-LSTM, by paying more attention to certain subsequences etc. Perhaps try to not relate what we do with enc-dec because it may be a bit confusing. Just use the example of how attention improves existing enc-dec models.}
% The attention strategies studied in this research are well-established state-of-the-art context-extraction models.
% \cw{Specifically, the following attention mechanisms are used to improve on the CNN-LSTM architecture mentioned in previous section} 
% % Specifically, the following existing attention strategies are recreated and combined with FCN and ResNet to experiment the aggregated performance for TSC.

% \begin{enumerate}[leftmargin=*]
%   \setlength\itemsep{0.2em}
%   \item Alignment Attention, introduced by Luong et. al. \cite{Luong2015-xr}
%   \item Bi-directional Attention, by Bahdanau et. al. \cite{Bahdanau2014-eh}
%   \item Locally and Globally focused Self-Attention Model, designed by Vaswani et. al. \cite{Vaswani2017-xw}
%   \item Multi-Head Attention Model, also by Vaswani et. al. \cite{Vaswani2017-xw}
% \end{enumerate}

% The next few sections describe the design features of the existing attention in regards to weakly labelled TSC. It is important to note, while almost all of the attention algorithms discussed in this study are integrated with FCN and ResNet, some of them are implemented independently to evaluate their standalone performance.

% \subsubsection{Luongs' Attention}

% % This research implements the attention from Luong et. al. along with CNN models (FCN and ResNet) and LSTM encoders and decoders for TSC. The algorithm was proposed by Luong et. al. for Seq-2-seq problems, but in this research, this algorithm is being used for TSC. 

% Since the original Luong et. al. \cite{Luong2015-xr} attention was designed for seq-2-seq models, this study implements the same architecture for time-series proposed by Huangwei \cite{Wieniawska2020-cv}.

% % In the original architecture, the model was built with twenty individual encoders and decoders. For this study, exactly four encoders and decoders are used such that in each batch, exactly four sequences are accepted and processed by the model. 

% % In every batch, the four input sequences are distributed to each of the four LSTM encoders in order. The idea is to classify the very last sequence based on the sequence-relevance information from the previous three sequences.

% % \begin{figure}[h]
% % \centering
% % \includegraphics[width=6cm]{.images/Luong.png}
% % \caption{Luongs' attention architecture to manage context}
% % \end{figure}

% % The encoders return a set of ‘hidden-states’ which are in fact feature-maps that are trained to understand and hold various features of the sequences. Since the last encoder hidden-state is responsible for the classification of the last (currently focused) sequence, this hidden-state is passed onto the decoder which repeats the vector four times to initiate a series of hidden decoder states.

% After receiving four sets of feature-maps from the CNN encoders, Luongs' attention creates an alignment-score vector. These alignment scores represent how well each of the first three subsequences match with the features extracted from the last subsequence. 

% The alignment score vector is multiplied with the encoder output for the last subsequence which is a method of identifying how much of the first 3 subsequences 'align' with the last subsequence. In other terms, this dot product generates a context vector, which is the weighted sum of the feature-maps of the last subsequence which are relevant to the previous subsequences.

% % But to get a decodable weight value, the alignment scores are again multiplied with the last hidden state from the encoder and a weighted sum is calculated. 

% Theoretically,  the LSTM decoder can use these weights to understands how well the last sequence is relevant to the previous sequences. This is done by concatenating this context vector with the CNN feature-maps to update the contextual information to the feature-maps.


% \subsubsection{Bi-directional Alignment Attention}

% Similar to Luongs' strategy, the attention concept proposed by Bahdanau et. al. is implemented to extract context of subsequences in order and reverse. The intuition behind using their algorithm is to understand the relevance of previous subsequences affecting the final one, and how the class of the previous subsequences could be affected based on the classification made on the final subsequence.

% % Following this concept of analysing data trends in both directions, this research implements a bi-directional encoder system on the existing Luongs' implementation to better understand the relevance of sequences. However, it is important to note that exactly four sequences are passed to this model per batch (similar to the previous implementation) to correctly classify the final sequence.

% % This attention model is implemented with a similar design as the previous model with some major changes in the encoders.

% \begin{figure}[h]
% \centering
% \includegraphics[width=7cm]{.images/BiDirectional.pdf}
% \caption{Bi-Directional attention for time-series}
% \end{figure}

% With the attention layers placed in between the encoders and decoders, the model begins by receiving a batch of four subsequence feature-maps. To allow analysis in both directions, this algorithm uses a bi-directional LSTM to learn the representation of the subsequences in order and backwards.

% Figure 3 illustrate how each direction of the bi-directional LSTM create a set of hidden states, labelled [E1, E2, E3, E4] for forward and [B1, B2, B3, B4] for backwards. Similar to Luongs' model, these hidden states represent the alignment scores of subsequences individually for each direction and hence, provides much more context for TSC.

% The algorithm then concatenates these hidden-states together, to allow each of them to collectively determine the overall alignment score of subsequences in both forward and backward directions. Receiving this updated context vector, the decoder combines it with the feature-maps from CNN to provide much more context than Luongs' model for TSC.

% % uses these sets of alignment scores to assign a weight of each of the first three sequences on the last one, representing how well the sequence follows features from the previous sequences.


% % \subsubsection{Transformers}

% % While the models by Luong et. al. \cite{Luong2015-xr} and Bahdanau et. al. \cite{Bahdanau2014-eh} can train and classify based on preceding sequences, two transformer designs, Self-Attention and Multi-Head Attention, are also evaluated in this research.

% % Both these transformer models \cite{Vaswani2017-xw} have built-in stacks of encoders and decoders, where each encoder is identical to the others and the same applies to the decoders. Generally, these encoders are designed as a bundle containing an Attention layer and a Feed-Forward Neural Network (FFNN). 


% % \begin{figure}[h]
% % \centering
% % \includegraphics[width=7cm]{.images/transformer.png}
% % \caption{Transformer Enc-Dec architecture}
% % \end{figure}


% % The Attention layer can be tweaked as necessary but generally, a Self-Attention layer (discussed later) is applied. The encoders and decoders contain internal residual connections, that are responsible for quick and adaptive feature extraction. The specific design features and advantages of this transformer architecture are further discussed in the next two sections where it is used within the Self-attention and Multi-Head Attention models.

% \subsubsection{Self-Attention}
% The core Self-Attention (SelfA) library implemented in this study was adapted from a Keras implementation by CyberZHG \cite{Zhao_undated-at}, built together with the CNN-LSTM encoders and decoders to allow TSC.

% The SelfA algorithm uses its internal complex 'Transformer' encoders-decoders to generate and maintain Query(Q), Key(K) and Value(V) vectors to keep track of context. Using the output from the CNN encoders, SelfA is expected to calculate the alignment scores through the Transformers (using a combination of attention and Feed-Forward Neural Networks). 

% SelfA is then expected to multiply these alignment scores with its initially created value(V) vector with certain calculations to flush out irrelevant values from context vector. In the case of weakly labelled time-series, this is expected to clean irrelevant context from the first three subsequences efficiently, to allow stronger matches to be found with the last subsequence.

% % and ignore any noise or redundancies of previous sequences that can affect the classification of the last one.

% % Firstly, the alignment score for each sequence is calculated and a softmax layer is used to normalise these series of alignment scores to reveal the weight of each sequence suited towards a particular category, also known as softmax scores. 

% % For each sequence, it multiplies the initially created value vector with the softmax scores. This creates a filter to extract the previous sequences that are more relevant to the current sequence than others, which are now completely diminished. This extra feature allows the model to flush out irrelevant previous sequences more smartly, and therefore ignore any noise or redundancies of previous sequences that can affect the classification of the last one.


% % The model can simply predict the category of each sequence based on the maximum softmax score for each sequence, but it proceeds to an additional step. 

% % The resulting scores can now be summed up to find the highest weight that corresponds to a category. However, 


% % The following part is important

% The SelfA algorithm also introduces the concept of `soft' vs. `hard' attention. In terms of TSC, soft attention creates a context vector of a window centred around the position of the current subsequence for maximum focus, and it stretches along the length of previous subsequences so the model gets an overall perspective of the context. On the contrary, hard attention aggressively focus on specific areas of input subsequences and therefore, identifies the relevance of definite sections of previous subsequence to the current. 

% This study implements both global and local SelfA algorithms, where global SelfA uses soft attention to learn overall patterns across the previous subsequences, and local SelfA uses a balance of soft and hard attention to extract alignment score for subsequences.

% This study also implements the two different alignment score functions proposed by the SelfA algorithm. The additive function calculates the scores by passing the context vectors to a Feed-Forward Network (FFN), whereas the multiplicative method pass the vectors into a softmax layer where the scores are calculated as the following equation.

% \begin{equation}Attention(Q, K, V)=softmax(\frac{QK^T}{\sqrt{d_k}})V\label{eq:1}\end{equation}

% For context extraction of subsequences, the additive function is expected to outperform multiplicative function, especially when the encoder key dimension, d\textsubscript{k}, is large. This d\textsubscript{k} value depends on the complexity of time-series subsequences, that is, the higher the number of features of the subsequence, the higher the dimensions and vice versa. In the case of multiplicative approach, large d\textsubscript{k} means large magnitudes of alignment scores are produced and therefore, extreme gradient values are generated which would negatively impact context extraction. For weakly labelled time-series, the number of features extracted from subsequences are expected to be high particularly due to additional noise and redundancies. However, assuming that the complexity is not definitive, this research evaluates SelfA strategy with both multiplicative and additive functions.

% The performance comparisons between global vs. local SelfA, and multiplicative vs. additive SelfA, are discussed later in section \ref{sec:performancediscussion}.


% \subsubsection{Multi-Head Attention}

% Finally, one of the most advanced Multi-Head Attention (MHA), proposed by  \cite{Vaswani2017-xw}, is a strategy which adopts the idea of self-attention previously discussed, but with more focused attention to various sections of previous subsequences in parallel.

% This algorithm runs several self-attention models together to perform context extraction, which make it computationally heavy. The MHA implemented in this study is primarily based on a Keras implementation by CyberZHG \cite{Zhao_undated-at}, with improvements made from the original implementation, which is available as a Tensorflow library \cite{noauthor_undated-sg}.

% % Together with the transformer encoders and decoders, the Multi-Head Attention implemented in this research can support weakly-labelled time-series classification.

% From the CNN encoders, MHA receives a set of four feature-maps per batch, again with the aim to classify the last one. This algorithm creates its initial vectors similar to SelfA but this is replicated `h’ times, where h is the number of heads selected as a hyper-parameter.

% % This h value decides how many self-attention models will be running in parallel where each self-attention receives its own set of K, V and Q vectors. The encoder designs are similar to SelfA encoders, however, the attention layer of the encoders in MHA will run ‘h’ parallel self-attentions within each encoder and a combined output of these will be passed into the next FFNN.

% % Each of the heads individually run dot-product self-attention, then concatenate all their K, V and Q vectors to a single set of each before passing them on. This ensures that each position within the encoder can attend to all positions of the previous layers, therefore building more context as it passes to the next encoder.

% \begin{figure}[h]
% \centering
% \includegraphics[width=8cm]{.images/MHA.pdf}
% \caption{MHA focus on time-series subsequence positions}
% \end{figure}

% In terms of TSC, MHA is expected to run the parallel Self-Attention encoders to understand the relevance of multiple areas of input subsequence at the same time. Figure 4 illustrates how MHA determines that the last subsequence is relevant to the two immediate-previous subsequences, but not to the first one. The multiple heads in MHA allows the model to focus on individual positions within these two previous subsequences to compare the various sections with the subsequence, and at the same time flushing out the irrelevant sections using self-attention as discussed before.

% While the multiple heads allow parallel focus on previous subsequences, it is important the the model considers the order. For TSC, it is only useful to keep track of neighbouring subsequences if they are part of a running trend. Nevertheless, MHA takes care of the order using an additional vector known as the positional encoding. Theoretically, this keeps track of the distance between each extracted context locations, giving the model a sense of subsequence order.

% MHA decoders are masked which means they will only consider previous subsequences. This is important in this study because it enables the model to suit real-time classifications where future subsequences are not known. While the previously discussed attention algorithms follow this restriction by default, MHA requires this additional masking due to multiple Self-Attention running in parallel and because MHA cannot centrally control the individual attention encoder/decoder positions.

% % As the model steps through all the decoders, a set of probability scores are returned from a softmax layer that helps the model determine which classification has the highest probability. This is very similar to the strategy followed by general self-attention models.


% \subsection{Multi-Step Models}

% Since the CNN-LSTM architecture is designed to receive four subsequences per batch, this study labels categorises these models as multi-step models. The list of the multi-step models implemented in this research are as follows.

% \begin{itemize}
%   \setlength\itemsep{0.2em}
%   \item \textbf{FCN\_LATTN}: Luong’s Attention with FCN
%   \item \textbf{ResNet\_LATTN}: Luong’s Attention with ResNet
%   \item \textbf{FCN\_BATTN}: Bahdanau’s Attention with FCN
%   \item \textbf{ResNet\_BATTN}: Bahdanau’s Attention with ResNet
%   \item \textbf{SelfA}: Local Additive Self-Attention
%   \item \textbf{FCN\_SelfA}: Local Additive Self-Attention with FCN
%   \item \textbf{FCN\_SelfA\_Global}: Global Self-Attention with FCN
%   \item \textbf{FCN\_SelfA\_Multiplicative}: Local Multiplicative Self-Attention with FCN
%   \item \textbf{ResNet\_SelfA}: Local Self-Attention with ResNet
%   \item \textbf{MHA}: Multi-Head Attention
%   \item \textbf{FCN\_MHA}: Multi-Head Attention with FCN
%   \item \textbf{ResNet\_MHA}: Multi-Head Attention with ResNet
% \end{itemize}


% \subsection{Single-Step Models}
% \cw{CW: I think the main reason for using single-step model is as a baseline. You can say that single-step models are when N=1 which then do not consider the relationship between the subsequences.}
% The multi-step models extract the features and context from the past three subsequences to predict the final one. 


% However, to evaluate the usefulness of extracting feature-maps and context within a single subsequence to predict its class, another set of models are built in this research. These models are designed to receive single subsequences per batch and are categorised as single-step models.

% The intuition behind the experimentation of these models is that each subsequence of time-series can show patterns within itself. For example, in the case of the EEG time-series, past three subsequences may show that the driver is continuously in a state of distraction and in the last subsequence, the first half of the subsequence continue distraction trends, but the second half may start revealing increasing driving concentration. The single-step models are designed to evaluate the performance on detecting these changes within single subsequences.

% The single-step models comprise of FCN and ResNet combined with MHA. Only the MHA algorithm is selected because of its ability to focus on various positions of a subsequence using parallel attention 'heads'. Each of these heads are expected to apply the self-attention strategy to different positions within the single subsequence to extract the context. Similar to the multi-step models, the CNN layers learn the features of the subsequence while the MHA layer simply adds the context vector.

% The single-step models implemented in this study are as follows.

% \begin{itemize}[leftmargin=*]
%   \setlength\itemsep{0.2em}
%   \item \textbf{LSA}: Luong’s Single-step Attention
%   \item \textbf{MHSA}: Multi-Head Single-step Attention
%   \item \textbf{FCN\_MHSA}: Multi-Head Single-step Attention with FCN
%   \item \textbf{ResNet\_MHSA}: Multi-Head Single-step Attention with ResNet
% \end{itemize}

% \section{Experimentation}
% \label{sec:experimentation}

% This section discusses how weakly labelled data is collected and prepared for evaluating the existing and proposed models in this study. It also describes the standard procedures maintained while testing the neural network models.

% \subsection{Experimental Setup}

% The models in this study are evaluated on the weakly labelled time-series dataset- Emotiv266 and EmotivRaw, supplied by the bioinformatics company Emotiv \cite{noauthor_undated-be}. The Emotiv dataset are collections of EEG brain signals data, captured using a light-weight and wireless Emotiv EPOC headset \footnote{\url{https://www.emotiv.com/epoc/}}, from 18 participants who undertook a 40 minute driving simulation and performed 16 different tasks (defined in Figure 1 legend) while driving. 

% In particular, the EmotivRaw dataset captures 14 individual EEG time-series in parallel, at a frequency of 128Hz (illustrated in Figure 1). As the participants perform various activities during driving, their brain activity alters and these are recorded in the EEG time-series. EmotivRaw has been spectrally transformed using Fast-Fourier transformation \cite{Oberst2007-dh}, and the metrics for each EEG channel were aggregated to allow additional parameters to be generated. In total, 266 parameters are created and combined to form Emotiv266. 

% \subsubsection{Data Preparation}

% Among the 16 participants, data from 12 randomly selected participants are used as the training set, another 2 as validation set and the remaining are used as test set to evaluate the models.

% EmotivRaw and Emotiv266 are long running lengths of multivariate time-series. To allow these time-series to be accepted by the deep-learning models, the long time-series was segmented into equally-sized 'subsequences', as shown in Figure 5.

% \begin{figure}[h]
% \centering
% \includegraphics[width=8cm]{.images/segmentation.pdf}
% \caption{Time-series segmentation of Emotiv266}
% \end{figure}

% For Emotiv266, these segmented subsequences are of dimensions 266 by 40, which refers to 266 parallel time-series of 40 time-steps in length. As Emotiv266 was updated at 4Hz, this length represent approximately 4 subsequences per second, which is a suitable simulation of a real-time stream. 

% % This study experiments with two sets of data, one with collections of four subsequences per batch to be consumed by the multi-step models, and the other with just one, to be consumed by the single-step models. 

% For the multi-step models of this study, this means that the four subsequences together represent a window-length of 160, designed such that attention can extract context from the first 120 samples (first three subsequences) to classify the final group of 40 samples (the last subsequence). The single-step models are given 1 subsequence per batch, which is of length 40.

% The subsequences are extracted as a sliding window with 50\% overlap. This is represented by a 'stride' value, which is kept at 20 (half of subsequence length) for Emotiv266.

% \subsubsection{Label Enhancements}

% While segmenting subsequences of 40 time-step during training, each of the time-step labels are compared. Within these 40 samples per subsequence, the majority label is mostly determined as the overall label of the subsequence, given as 0 or 1 corresponding to distracted or focused driving respectively. However, if there are two different groups of labels across the subsequence, the 40 time-step window is split into two and each is filled with insignificant placeholder values to fill each window size to 40. This ensures that each subsequence now has consistent labels. If the window has over two label variations (which is unlikely in Emotiv), the windows are discarded. This eliminates any negative impact in TSC experimentation that can be caused by the segmentation.

% \subsubsection{Up-sampling}

% Since data for distracted driving is difficult to capture, the Emotiv dataset are highly imbalanced. The majority label is `focused' driving, which is almost twice the number of `distracted' data (a ratio of 3828 to 2032 samples). Although the attention models are expected to mitigate the effect of imbalanced data, this study adds the option to up-sample the data before running the models. The effect of up-sampling data on the performance of the models of this study is analysed in detail later in the results section.

% A python library ‘imblearn’ \cite{noauthor_undated-dl} is used to repeatedly duplicate random records from the minority group (distracted category). This equalises the number of records for each label and provides a fair learning opportunity for the models.

% \subsection{Experimenting Models}

% % In this section, the proposed attention approaches are evaluated on the benchmark dataset Emotiv266 and EmotivRaw. This, and the next few sections discusses the impacts of the attention models and identifies various performance benefits and drawbacks of each model for weakly-labelled time-series classification. 

% When all the models are experimented in this study, it is important to note that they are fitted with an ADAM optimiser \cite{Kingma2014-nu}, and the categorical cross-entropy is used to determine the loss per epoch. A script, available with the code  \footnote{\url{https://github.com/Surayez/EmotivDriverDistraction}}, runs each model five times with one hundred epochs each, enabling the ability to take average of performance.

% The models are also programmed to reduce the learning rate as the loss gradient begins to flatten. This ensures the model can reach a minimum plateau in validation loss, and hence perform TSC with minimum loss. Moreover, the experiments are designed to minimise empirical risk by selecting the best models with minimum loss among the epochs.

% % After running classification, the models output their performance accuracy, AUC (Area Under the Curve) and F1 scores are used as primary metrics to evaluate each model, and these metrics are compared to the existing approaches.

% Table 1 outlines the average validation scores of each of the models running on Emotiv266 and EmotivRaw. The models are trained on training set and the metrics in this table are the results of evaluating the models on test set.

% \input{main_results_table}

% \section{Performance Analysis}
% \label{sec:performancediscussion}

% \subsection{Accuracy}

% Immediately noticeable from Table 1, most of the attention implementations perform with higher accuracies than the existing deep learning models. The addition of the LSTM layer, for basic context relevance, improved the accuracy scores of FCN by 5 per cent and ResNet by 7 per cent, which is a little higher than the accuracy by achieved by ROCKET.

% However, the most notable models include FCN\_SelfA, MHA and FCN\_MHA, which show significant improvements in classification accuracy. On average, FCN\_SelfA, classifies approximately 13 per cent more accurately compared to the existing FCN model and over 7 per cent than FCN\_LSTM on Emotiv266. Following this, FCN\_MHA and MHA perform with over 10 per cent higher accuracies than FCN, and 4 per cent higher accuracies when compared to FCN\_LSTM. These are dramatic improvements in weakly labelled TSC, in comparison to the existing models.

% In fact, the accuracy scores of SelfA and MHA by themselves are surprisingly high. It indicates that the position based context extraction of SelfA and MHA can solely perform TSC more accurately on weakly labelled data than the existing models. However, the high loss metrics of these two models, discussed later, indicate that this is not always the case.

% The simpler LATTN and BATTN models also demonstrate improved the accuracy of TSC. In comparison to existing models, FCN\_LATTN and FCN\_BATTN show almost 5 per cent improvement, but when considered with FCN\_LSTM which is almost the same, the additional attention algorithm is not improving the performance significantly. This is largely due to underfitting, and this is discussed in detail in a later section.

% \subsection{AUC}

% To further establish the improvement using attention algorithms, the AUC scores are evaluated as part of this analysis. AUC scores are important for this binary classification evaluation as it eliminates the effect of bias in the target categories when comparing the average performance of classification algorithms \cite{Huang2005-bn}. 

% The attention models clearly demonstrate significant improvements in AUC metrics. FCN\_MHA performs with an almost 5 per cent higher AUC score compared to the FCN model, which has the highest AUC score among the existing TSC models. Similarly, FCN\_SelfA shows approximately 3 per cent improvement than FCN. Even when LSTM extracts the basic context, it improves the AUC by almost 2 per cent. This demonstrates that the higher accuracy scores of FCN are, in fact, improving the overall performance of TSC.

% On the other hand, the ResNet models show much lower AUC scores in comparison to FCN models. This indicates that the accuracy improvements when using attention with ResNet may not be improving the overall performance of the models. The primary reason for this is that ResNet is overfitting the training data, and this issue is discussed in detail in a later section.

% \subsection{F1}
% The F1 scores of each model are important in this study because the initial Emotiv data is highly imbalanced. Table 1 shows the maximum average F1 score among the existing models is at 54 per cent achieved by ROCKET. Although FCN\_SelfA and FCN\_MHA improved the F1 score by almost 4 per cent when compared to FCN, this is not a drastic improvement considering the F1 score by ROCKET is around the same.

% However, the usefulness of attention, with regards to F1 score, is reflected when the models are evaluated with imbalanced data. Table 2 compares the F1 and accuracy scores by the existing FCN and ResNet, and the attention model with highest accuracy from Table 1, FCN\_SelfA, before and after the training set of Emotiv266 is up-sampled.

% \input{upsample-results}

% Table 2 shows that the accuracy and F1 driving scores of FCN and ResNet are quite high when the data is imbalanced. However, the F1 distracted score is significantly low which means that the models can accurately classify most of the driving (dominant) subsequences, but only few of the distracted (minor) category. The overall accuracy is high due to the higher true positives where in reality, most of the distracted category classifications are incorrect.

% Again when the data is up-sampled (balanced), the number of accurate distracted classifications improve, hence the distracted F1 scores rise sharply. Now that FCN and ResNet are equally false-classifying for both categories, the overall accuracy falls.

% Nevertheless, the F1 metrics of FCN\_SelfA state that the effect of up-sampling has a minor effect on both the accuracy and F1 scores for driving. Moreover, the difference between the distracted F1 scores before and after up-sampling is much smaller than in the case of FCN and ResNet. This proves that the attention strategy, is assisting the FCN model to make better decisions of the minor category as expected. Using the context information from previous subsequences, it is able to eliminate the effect of imbalanced data. Therefore, it is safe to say that the improved accuracy of FCN\_SelfA would be preserved even when the input time-series is imbalanced, as in a real-world setting.


% \subsection{Validation Loss}

% Although there is an increase in overall accuracy, the loss graphs generated by the FCN\_SelfA and FCN\_MHA models indicate overfitting of training set. This is identified by the fluctuating validation loss while the training loss decrease exponentially.

% % The issue is that the complex encoder-decoder architecture of SelfA and MHA make these models over-confident on the training set. 
% Due to overfitting, when the models are given validation set, the false predictions are heavily penalised by significantly increasing loss and correct predictions have minor effect on decreasing the loss \cite{Salman2019-at}. This explains the behaviour of Self-Attention and MHA classifying with high accuracy but also with higher loss.

% On the contrary, LATTN and BATTN models have a better loss pattern despite their minor improvements in accuracy. Each of its validation loss shows exponential decrease, similar to its training loss. Once again, this is a typical indication that the models are underfitting the training data, and is discussed in a later section.
% % An underfit by the attention layers mean that the attention layer is not extracting enough contextual information to have any significant effect on the performance of the model.


% \subsection{Effect of Overfitting}

% Figure 6 shows the training, validation and test accuracies in a sample evaluation of the models on the Emotiv266 time-series. It is quite clear that almost all the models have a much higher training accuracy than test accuracy, which identifies that the models are largely overfitting the training set.

% The reason for this behaviour is due to the complex architectures of FCN and ResNet. When these models are training on a weakly labelled dataset before attention is applied, they learn the noise and redundancies of the training data too accurately. This clouds their judgement of the noise as distinctive features of subsequences. As the models are then evaluated on test data, they fail to identify the new patterns of noise and redundancies in test set, leading to low test accuracies.

% As expected, the attention layers significantly improve the accuracy of the models by cutting down this effect. The improved results indicate that attention can successfully support TSC by extracting context of subsequences. However, this effect is not completely eliminated.

% \begin{figure}[h]
% \centering
% \includegraphics[width=8cm]{.images/model_accuracies.pdf}
% \caption{Accuracy of TSC models with 100 epochs}
% \end{figure}


% \subsection{Effect of Underfitting}

% The performance of LATTN and BATTN show some improvements compared to existing models, however, the accuracy and validation loss metrics suggests that these models are underfitting the training set.

% Attention algorithms by Luong et. al. and Bahdanau et. al. are considering subsequence relevance information because it shows minor improvements, but the simplicity of the alignment calculation algorithm fails to retrieve enough context in comparison to SelfA or MHA. The more complex internal encoders and decoders of SelfA and MHA provide them with powerful computational support to 'attend’ more sections within the previous subsequences, and therefore better alignments to be found.

% Nevertheless, LATTN and BATTN were re-evaluated on longer epochs (300 epochs) with the expectation further training may eliminate the effect of underfitting. Unfortunately, the performance did not improve even with the longer training period.


% \subsection{FCN and ResNet}

% The performance evaluations of this study indicate that ResNet has inconsistent improvements with LSTM and attention algorithms. Table 1 shows that ResNet performs well when combined with SelfA and BATTN, but show lower improvements with MHA and LATTN. The overall accuracy metrics suggest that FCN is performing significantly better with additional context information than ResNet.

% However, the reason for this behaviour can be pointed to the more complex architecture of ResNet. The feature-maps returned from 3 convolution blocks of FCN, seems to be better interpreted by attention, than with that from 9 convolution blocks of ResNet. Because of this, ResNet overfits the training set slightly more than FCN and it is reflected in the results table.


% \subsection{Single-Step Models}

% When this study evaluated the single step models on Emotiv dataset, they did not demonstrate exceptional performance metrics. The results from Table 1 indicate that the single-step models improve TSC when compared to FCN and ResNet, but not as much as the multi-step models.

% This suggests that understanding the context of various positions within the single subsequence is not enough to minimise the effect of weakly labelled data in Emotiv time-series. The attention models examining a larger window for context (multi-step models) are performing much better. 

% However, these performance metrics do not disqualify the single-step models from weakly labelled TSC. Intuitively, the models are expected to prove very useful when subsequences of time-series are of higher lengths and show more repetitive pattern. For the case of Emotiv266 or EmotivRaw, each subsequence block is not exceptionally long to take advantage of such context analysis and therefore, the single-step models show insignificant improvements compared to the existing models.


% \subsection{Global vs. Local SelfA}

% SelfA is one of the best performing models of this study and further analysis are conducted to explore SelfA for TSC.

% Firstly, this research evaluates the performance of global and localised SelfA algorithms against Emotiv266 with same training and validation sets. As discussed earlier, local SelfA is expected to be more accurate for Emotiv266 because it considers various positions within previous subsequences, rather than a global `soft' focus. The results are consistent with the expectations as local SelfA performed 4 per cent more accurately than global SelfA on average.

% \subsection{Additive vs. Multiplicative SelfA}

% Furthermore, the performance of additive and multiplicative SelfA are evaluated on the same dataset as before. When local FCN\_SelfA is evaluated with the additive alignment function, it performed 5 per cent more accurately than when evaluated with multiplicative alignment function.

% The reason for this performance difference is the previously discussed FFN layer, which is present in the additive algorithm but is replaced with a softmax calculation\eqref{eq:1} in the multiplicative algorithm. Due to the noise and data redundancies, the subsequences in Emotiv are of high complexities. The extra FFN layer helps the additive model interpret the encoder keys with larger dimensions of the Emotiv subsequences, and causes the multiplicative calculation to produce extreme gradient values which negatively impact context extraction.


% \subsection{Effect of normalisation}

% Table 3 shows the average outcomes when the models are evaluated on time-series with:
% \begin{itemize}[leftmargin=*]
%   \setlength\itemsep{0.1em}
%   \item No normalisation
%   \item Only normalisation during sub-sequence extraction
%   \item Only normalisation during series extraction
%   \item Both normalisation as above
% \end{itemize}

% \input{normalisation_results}

% While it is a standard practice to normalise time-series for TSC using deep-learning, the performance of the models without the two type of normalisation applied in this study is evaluated to further reinforce the TSC improvements using attention. The outcomes in Table 3 highlights the improved performance using attention by both Self-Attention and Multi-Head Attention models.


% \section{Conclusion}
% From the experiments on the real-world Emotiv dataset, it can be concluded that the attention strategy improves the performance of existing state-of-the-art TSC algorithms on weakly-labelled time-series. To eliminate the effect of weak-labelled time-series from the real-world setting, the extraction and interpretation of subsequence context information help supervised CNN to improve their performance of subsequence classification. In particular, the performance of Self-Attention with FCN (with additive function in localised context) and Multi-Head Attention with FCN displays the most dramatic improvements, and can therefore be concluded as the top models of this study.

% The set of models developed as part of this research can complement any further studies for real-time TSC. The CNN encoders and LSTM decoders architecture can be used to further analyse the performance of these models on dataset from different domains.

% %\end{document}  % This is where a 'short' article might terminate


% % %ACKNOWLEDGEMENTS are optional
% % \section{Acknowledgements}
% % This section is optional; it is a location for you
% % to acknowledge grants, funding, editing assistance and
% % what have you.  In the present case, for example, the
% % authors would like to thank Gerald Murray of ACM for
% % his help in codifying this \textit{Author's Guide}
% % and the \textbf{.cls} and \textbf{.tex} files that it describes.

% %
% % The following two commands are all you need in the
% % initial runs of your .tex file to
% % produce the bibliography for the citations in your paper.
% \bibliographystyle{abbrv}
% \bibliography{sigproc}  % sigproc.bib is the name of the Bibliography in this case
% % You must have a proper ".bib" file
% %  and remember to run:
% % latex bibtex latex latex
% % to resolve all references
% %
% % ACM needs 'a single self-contained file'!
% %
% %APPENDICES are optional
% % SIGKDD: balancing columns messes up the footers: Sunita Sarawagi, Jan 2000.
% % \balancecolumns
% \appendix

% \section{Self-Attention Comparisons}

% \begin{figure}[h]
% \centering
% \includegraphics[width=7cm]{.images/selfa_FCN_vs_selfa_FCN_Global.png}
% \caption{Accuracy of Global vs. Local SelfA}
% \end{figure}


% \begin{figure}[h]
% \centering
% \includegraphics[width=7cm]{.images/additive_vs_multiplicative_sefl_Attn.png}
% \caption{Accuracy of Additive vs. Multiplicative SelfA}
% \end{figure}

% \section{Validation Loss Graphs}
% \cw{CW: If we are not using them, then we should remove these graphs from the appendix and paper}
% \begin{figure}[h]
% \centering
% \includegraphics[width=6cm]{.images/epochs_loss_fcn_lstm.png}
% \caption{Epoch loss of FCN\_LSTM}
% \end{figure}

% \begin{figure}[h]
% \centering
% \includegraphics[width=6cm]{.images/epochs_loss_ResNet_LSTM.png}
% \caption{Epoch loss of ResNet\_LSTM}
% \end{figure}

% \begin{figure}[h]
% \centering
% \includegraphics[width=6cm]{.images/epochs_loss_SelfA_FCN.png}
% \caption{Epoch loss of FCN\_SelfA}
% \end{figure}

% \begin{figure}[h]
% \centering
% \includegraphics[width=6cm]{.images/epochs_loss_MHA_FCN.png}
% \caption{Epoch loss of FCN\_MHA}
% \end{figure}

% \begin{figure}[h]
% \centering
% \includegraphics[width=6cm]{.images/epochs_loss_LATTN_FCN.png}
% \caption{Epoch loss of FCN\_LATTN}
% \end{figure}

% \begin{figure}[h]
% \centering
% \includegraphics[width=6cm]{.images/epochs_loss_BATTN_FCN.png}
% \caption{Epoch loss of FCN\_BATTN}
% \end{figure}




% % %Appendix A
% % \section{Headings in Appendices}
% % The rules about hierarchical headings discussed above for
% % the body of the article are different in the appendices.
% % In the \textbf{appendix} environment, the command
% % \textbf{section} is used to
% % indicate the start of each Appendix, with alphabetic order
% % designation (i.e. the first is A, the second B, etc.) and
% % a title (if you include one).  So, if you need
% % hierarchical structure
% % \textit{within} an Appendix, start with \textbf{subsection} as the
% % highest level. Here is an outline of the body of this
% % document in Appendix-appropriate form:
% % \subsection{Introduction}
% % \subsection{The Body of the Paper}
% % \subsubsection{Type Changes and Special Characters}
% % \subsubsection{Math Equations}
% % \paragraph{Inline (In-text) Equations}
% % \paragraph{Display Equations}
% % \subsubsection{Citations}
% % \subsubsection{Tables}
% % \subsubsection{Figures}
% % \subsubsection{Theorem-like Constructs}
% % \subsubsection*{A Caveat for the \TeX\ Expert}
% % \subsection{Conclusions}
% % \subsection{Acknowledgements}
% % \subsection{Additional Authors}
% % This section is inserted by \LaTeX; you do not insert it.
% % You just add the names and information in the
% % \texttt{{\char'134}additionalauthors} command at the start
% % of the document.
% % \subsection{References}
% % Generated by bibtex from your ~.bib file.  Run latex,
% % then bibtex, then latex twice (to resolve references)
% % to create the ~.bbl file.  Insert that ~.bbl file into
% % the .tex source file and comment out
% % the command \texttt{{\char'134}thebibliography}.
% % % This next section command marks the start of
% % % Appendix B, and does not continue the present hierarchy
% % \section{More Help for the Hardy}
% % The acmproc-sp document class file itself is chock-full of succinct
% % and helpful comments.  If you consider yourself a moderately
% % experienced to expert user of \LaTeX, you may find reading
% % it useful but please remember not to change it.

% % That's all folks!


% \end{document}

